Is Decentralized Finance Actually Decentralized? An Interdisciplinary Framework Integrating Network Theory, Agent-Based Simulation, and Longitudinal Evidence from Aave, GHO Issuance, and Cross-Chain Expansion

Decentralized finance (DeFi) can broaden access while leaving activity, network position, and infrastructure concentrated. We develop a four-dimensional framework for participation, activity distribution, structural position, and infrastructure dependence, integrating network theory, theorem-consistent agent-based simulation, and longitudinal analysis of 1,956,216 Aave V3 Pool events. We study GHO issuance on Ethereum (15 July 2023) and its first cross-chain expansion to Aave's existing Arbitrum market (2 July 2024). Excluding each activation week, mean weekly active position-holder addresses increased by 91.0% around Ethereum issuance and 1.7% around Arbitrum expansion, while activity concentration fell by 31.5% on Ethereum but rose by 58.1% on Arbitrum. On a common 2024 calendar, the Arbitrum--Gnosis DiD-style change is +1.9833 for log participation and -0.01842 for position-holder-event HHI. Rule-based simulations recover the analytical equilibrium and show why aggregate growth can coexist with lower, unchanged, or higher concentration, while chain dispersion alone cannot establish route or shared-component resilience. Role-aware analysis further shows that network-structure conclusions vary by protocol action and scale. Intellectually, the framework explains why four dimensions of decentralization can diverge. Practically, it helps researchers, protocol designers, governance communities, and policymakers assess stablecoin growth without equating adoption with decentralization.

==> figures/fig02c_literature_method_evidence.tex <==
\begin{figure}[!htbp]
\centering
\suspendrefereelines
\includegraphics[width=0.98\textwidth]{generated/figures/fig_literature_method_evidence_map.pdf}
\resumerefereelines
\caption{Count-preserving method--domain--evidence Sankey for the fixed 18-work literature-coding audit corpus. Each work is assigned one method family, research domain, and evidence-object family using the documented coding rules. Node heights and ribbon widths encode numbers of works, and every middle node conserves inflow and outflow. Colour follows the method family so split paths remain traceable across both stages. Paper-level assignments and aggregate node and link tables accompany the figure. The fixed corpus tests coding traceability; it is not an exhaustive review and does not include every recent source discussed in Section~\ref{subsec:literature}. Ribbons denote author-coded scope relations only, not citation, influence, agreement, intellectual descent, or empirical support for an Aave-specific mechanism.}
\label{fig:literature-method-evidence}
\end{figure}


==> generated/tables/policy_events.tex <==
\begin{table}[t]
\caption{Verified protocol-policy event registry used to define candidate treatments.}
\label{tab:policy-events}
\centering
\AVTableSetup
\begin{tabularx}{\textwidth}{P{2.45cm}P{2.05cm}P{2.05cm}Y P{2.05cm}}
\toprule
\AVTableHeader
\textbf{Event} & \textbf{Unit} & \textbf{Activation clock} & \textbf{Economic mechanism} & \textbf{Evidence status} \\
\midrule
GHO mainnet launch & Aave Ethereum & 2023-07-15 & Native stablecoin adds borrowing and DAO revenue & Locked A+ \\
Cross-chain GHO on Arbitrum & Arbitrum GHO & 2024-07-02 & CCIP access adds bridge and facilitator dependence & Locked A+ \\
\bottomrule
\end{tabularx}
\begin{tablenotes}\AVTableNoteFont
\item \emph{Notes:} Announcement, execution, technical readiness, first use, and publicity are separate records. Primary clocks use successful governance execution; exact blocks and UTC timestamps remain in the event-source audit.
\end{tablenotes}
\end{table}


==> generated/tables/simulation_mechanism_check.tex <==
\begin{table}[t]
\caption{Stylized network-game mechanism check at the reference parameter set.}
\label{tab:simulation-mechanism}
\centering
\AVTableSetup
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
\AVTableHeader
& \multicolumn{2}{c}{\textbf{Breadth and scale}} & \multicolumn{3}{c}{\textbf{Concentration}} & \textbf{Resilience} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(l){7-7}
\textbf{Scenario} & $N_{+}$ & $X/X_{0}$ & $H_x$ & $H_c$ & $H_s$ & $L_{\max}$ \\
\midrule
Baseline & 96 & 1.000 & 0.014 & 1.000 & 0.012 & 0.000 \\
GHO issuance & 166 & 2.150 & 0.008 & 1.000 & 0.007 & 0.000 \\
One route & 191 & 2.740 & 0.007 & 0.501 & 0.006 & 0.477 \\
Two routes & 191 & 2.740 & 0.007 & 0.501 & 0.006 & 0.238 \\
\bottomrule
\end{tabular*}
\begin{tablenotes}\AVTableNoteFont
\item \emph{Notes:} Deterministic synthetic mechanism check with $\beta=0.50$. $N_{+}$ is active entities; $X/X_0$ is activity relative to the benchmark; $H_x$, $H_c$, and $H_s$ are activity, chain, and structural HHI; $L_{\max}$ is the activity share lost with the largest route. Values are not empirical estimates.
\end{tablenotes}
\end{table}


==> release/figures/fig02c_literature_method_evidence.tex <==
\begin{figure}[!htbp]
\centering
\suspendrefereelines
\includegraphics[width=0.98\textwidth]{generated/figures/fig_literature_method_evidence_map.pdf}
\resumerefereelines
\caption{Count-preserving method--domain--evidence Sankey for the fixed 18-work literature-coding audit corpus. Each work is assigned one method family, research domain, and evidence-object family using the documented coding rules. Node heights and ribbon widths encode numbers of works, and every middle node conserves inflow and outflow. Colour follows the method family so split paths remain traceable across both stages. Paper-level assignments and aggregate node and link tables accompany the figure. The fixed corpus tests coding traceability; it is not an exhaustive review and does not include every recent source discussed in Section~\ref{subsec:literature}. Ribbons denote author-coded scope relations only, not citation, influence, agreement, intellectual descent, or empirical support for an Aave-specific mechanism.}
\label{fig:literature-method-evidence}
\end{figure}


==> release/figures/fig05_real_v5_cross_chain.tex <==
% Authoritative visual: scripts/render_svis_upgrade.py.
\begin{figure}[!htbp]
\centering
\suspendrefereelines
\includegraphics[width=0.98\textwidth]{generated/figures/fig_multidimensional_trajectories.pdf}
\resumerefereelines
\caption{Four complementary address-level trajectories around chain-specific institutional clocks. Panel A indexes each chain's weekly active position-holder-address count to its own mean over weeks $-16$ to $-1$. Panel B reports the HHI of equally weighted Pool-event frequency, where larger values indicate greater concentration. Panel C reports the share of Pool events assigned to the top 10\% of active position-holder addresses, and Panel D reports the minimum number of active position-holder addresses needed to reach 51\% of events. The vertical dashed line marks week 0 and light shading marks post-clock weeks. Ethereum and Arbitrum use different verified clocks and different calendar years; the lines are descriptive trajectories, not a treated--control comparison. All actions and reserves are aggregated, addresses are not verified economic actors, and no GHO-specific or causal effect is shown.}
\label{fig:real-v5-cross-chain}
\end{figure}


==> release/figures/fig05b_action_layer_profile.tex <==
% Authoritative visual: scripts/render_svis_upgrade.py.
\begin{figure}[!htbp]
\centering
\suspendrefereelines
\includegraphics[width=0.98\textwidth]{generated/figures/fig_action_layer_profile.pdf}
\resumerefereelines
\caption{Action-layer topology profile for the audited Pool-event system. Rows separate Supply, Withdraw, Borrow, Repay, and Liquidation on Ethereum and Arbitrum; columns report event scale, self-directed-event share, action-side and position-holder-side strength HHI, the scale-adjusted effective PageRank-node fraction, and maximum-$k$-core node share. Printed values are the estimands; cell color is normalized separately within each column and supports comparison of visual rank only. Withdraw is fully self-directed under the decoded role map, so removing self-loops leaves no delegated topology and the PageRank fraction is not applicable. Layers reuse the same address namespace, but the available compact output contains neither verified interlayer edges nor bridge-route flows. The figure therefore compares typed intralayer summaries and does not claim a multiplex community, economic-actor, or route-dependence result.}
\label{fig:action-layer-profile}
\end{figure}


==> release/figures/fig05c_centrality_roles.tex <==
% Authoritative visual source: generated/render_svis_upgrade.py and editable SVG.
\begin{figure}[!htbp]
\centering
\suspendrefereelines
\includegraphics[width=0.98\textwidth]{generated/figures/fig_centrality_roles.pdf}
\resumerefereelines
\caption{Global centrality dispersion coexists with small operational cores and role-specific high-coreness tails. Panel A reports the full-graph address shares in the maximum-$k$ core, the fitted Borgatti--Everett (BE) core, and any weekly maximum core on a logarithmic scale. Ethereum is shown with solid navy bars and Arbitrum with hatched slate bars; each value is printed directly above its bar. The two-node BE solutions equal the algorithmic lower bound. Panel B compares the full-graph role composition with roles at or above each chain's 99th percentile of Rombach coreness; blue, orange, and teal denote position-holder, action-side, and dual-role semantics. The effective PageRank-node fractions remain 99.41\% on Ethereum and 98.01\% on Arbitrum, so the figure focuses on the local-core and role evidence that qualifies that diffuse global mass. Statistics use all 8,891 Ethereum and 50,693 Arbitrum address-role nodes, not the 160-node display backbone. Address roles do not establish ownership or independent economic actors, and neither panel is a causal, dynamic-network, or removal-dependence estimate.}
\label{fig:centrality-roles}
\end{figure}


==> release/figures/fig05d_address_state_flows.tex <==
\begin{figure}[t]
\centering
\suspendrefereelines
\includegraphics[width=0.98\textwidth]{generated/figures/fig_address_state_flows.pdf}
\resumerefereelines
\caption{Observed adjacent-week position-holder-address state evolution. Panels A and B decompose each current weekly active set into addresses retained from the previous week and entrants; exits from the previous active set are plotted below zero, and the dark line is the current active total. Thus, for week $t$, entrants plus retained addresses equal the current active count, while exits plus retained addresses equal the week-$t-1$ active count. Panels C and D report entrants as a share of the current active set and retained and exiting addresses as shares of the prior active set. Week $-16$ has no prior-week rate and is omitted from the rate panels. The dashed line marks week 0 and shading marks post-clock weeks. Ethereum and Arbitrum use different verified clocks and calendar years; all actions and reserves are aggregated. These are address-set membership transitions, not people, value transfers, bridge-route flows, cross-chain movements, GHO-specific effects, or causal estimates.}
\label{fig:address-state-flows}
\end{figure}


==> release/figures/fig07_arbitrum_gnosis_comparative_dynamics.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{generated/comparison/fig_arbitrum_gnosis_comparative_dynamics.pdf}
\caption{Arbitrum--Gnosis comparative dynamics around the 2 July 2024 GHO expansion. Panels A/D show observed weekly log participation and position-holder-event HHI; B/E show controlled interrupted-time-series fits to the Arbitrum-minus-Gnosis gap; and C/F show gaps centered on their clean-pre means. Purple shading marks the excluded anticipation window ($-8$ to $-1$) and grey marks excluded week 0. Fitted segments stop at the included clean-pre ($-16$ to $-9$) and post ($+1$ to $+16$) boundaries; the dashed line is the clean-pre no-change projection. Week-0 level shifts are extrapolated across the omitted interval. These are comparative longitudinal estimates with descriptive HAC uncertainty, not identified treatment effects.}
\label{fig:arbitrum-gnosis-comparative-dynamics}
\end{figure*}


==> release/figures/figA_display_community_audit.tex <==
\begin{figure}[t]
\centering
\suspendrefereelines
\includegraphics[width=0.98\textwidth]{generated/figures/fig_display_community_audit.pdf}
\resumerefereelines
\caption{Community sensitivity analysis on the fixed display backbones. Panels A and B color the 160 displayed nodes per chain by a weighted greedy-modularity partition of the top-weight backbone; community identifiers are size-ranked and chain-local, orange rings mark maximum-$k$-core nodes, violet diamonds mark the two-node Borgatti--Everett core, node size encodes PageRank, and faint edges are the displayed relations. Panel C reports community counts and modularity $Q$ after applying raw, $\log(1+w)$, or binary edge weights. Panel D reports normalized mutual information (NMI) between the raw-weight partition and each alternative. The visible changes under weight definitions are the result: community assignments on this compact backbone are specification-sensitive. The figure is a display-subset diagnostic, not a partition of the complete directed weighted graphs, a temporal-community estimate, an economic-actor grouping, or an estimation sample. Full-graph community and persistence claims require the complete edge-event table and corresponding validation checks.}
\label{fig:display-community-audit}
\end{figure}


==> release/generated/simulation/simulation_results_macros.tex <==
% Generated by run_mvp.py; do not edit manually.
\newcommand{\SimIterWeak}{18}
\newcommand{\SimIterStrong}{79}
\newcommand{\SimIterNear}{438}
\newcommand{\SimMaxAnalyticError}{1.90e-08}
\newcommand{\SimChainHHI}{0.52}
\newcommand{\SimPeripheralActivity}{+14.78\%}
\newcommand{\SimPeripheralHHI}{-4.17\%}
\newcommand{\SimProportionalActivity}{+18.85\%}
\newcommand{\SimProportionalHHI}{-0.00\%}
\newcommand{\SimIncumbentActivity}{+26.34\%}
\newcommand{\SimIncumbentHHI}{+4.77\%}


==> release/generated/simulation/simulation_results_table.tex <==
% Generated by run_mvp.py; do not edit manually.
\begin{table}[t]
\centering
\caption{Theorem-to-simulation checks and evidence boundaries.}
\label{tab:theory-simulation-results}
\AVTableSetup
\begin{tabularx}{\textwidth}{P{0.18\textwidth}P{0.27\textwidth}P{0.27\textwidth}Y}
\toprule
Analytical result & Synthetic experiment & Verified numerical pattern & Evidence boundary \\
\midrule
Network amplification & Central benefit shock at $\kappa=0.25,0.75,0.95$ & 18, 79, and 438 iterations; maximum stable analytical error 1.90e-08 & Fixed synthetic network; no participant entry \\
Growth--concentration divergence & Equal-mass peripheral, proportional, and incumbent allocations & Peripheral expansion: $\Delta X=+14.78\%$, $\Delta H_x=-4.17\%$; Proportional: $\Delta X=+18.85\%$, $\Delta H_x=-0.00\%$; Incumbent amplification: $\Delta X=+26.34\%$, $\Delta H_x=+4.77\%$ & Ten synthetic seeds; fixed active set \\
Chain dispersion versus resilience & Identical 60/40 chain shares with alternative route/component structures & Chain HHI $0.52$ throughout; worst route loss $40\%,20\%,10\%,10\%$; shared-component loss reaches $40\%$ in the final case & Static synthetic stress construction, not observed bridge failure \\
\bottomrule
\end{tabularx}
\end{table}


==> release/generated/tables/policy_events.tex <==
\begin{table}[t]
\caption{Verified protocol-policy event registry used to define candidate treatments.}
\label{tab:policy-events}
\centering
\AVTableSetup
\begin{tabularx}{\textwidth}{P{2.45cm}P{2.05cm}P{2.05cm}Y P{2.05cm}}
\toprule
\AVTableHeader
\textbf{Event} & \textbf{Unit} & \textbf{Activation clock} & \textbf{Economic mechanism} & \textbf{Evidence status} \\
\midrule
GHO mainnet launch & Aave Ethereum & 2023-07-15 & Native stablecoin adds borrowing and DAO revenue & Locked A+ \\
Cross-chain GHO on Arbitrum & Arbitrum GHO & 2024-07-02 & CCIP access adds bridge and facilitator dependence & Locked A+ \\
\bottomrule
\end{tabularx}
\begin{tablenotes}\AVTableNoteFont
\item \emph{Notes:} Announcement, execution, technical readiness, first use, and publicity are separate records. Primary clocks use successful governance execution; exact blocks and UTC timestamps remain in the event-source audit.
\end{tablenotes}
\end{table}


==> release/generated/tables/simulation_mechanism_check.tex <==
\begin{table}[t]
\caption{Stylized network-game mechanism check at the reference parameter set.}
\label{tab:simulation-mechanism}
\centering
\AVTableSetup
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
\AVTableHeader
& \multicolumn{2}{c}{\textbf{Breadth and scale}} & \multicolumn{3}{c}{\textbf{Concentration}} & \textbf{Resilience} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(l){7-7}
\textbf{Scenario} & $N_{+}$ & $X/X_{0}$ & $H_x$ & $H_c$ & $H_s$ & $L_{\max}$ \\
\midrule
Baseline & 96 & 1.000 & 0.014 & 1.000 & 0.012 & 0.000 \\
GHO issuance & 166 & 2.150 & 0.008 & 1.000 & 0.007 & 0.000 \\
One route & 191 & 2.740 & 0.007 & 0.501 & 0.006 & 0.477 \\
Two routes & 191 & 2.740 & 0.007 & 0.501 & 0.006 & 0.238 \\
\bottomrule
\end{tabular*}
\begin{tablenotes}\AVTableNoteFont
\item \emph{Notes:} Deterministic synthetic mechanism check with $\beta=0.50$. $N_{+}$ is active entities; $X/X_0$ is activity relative to the benchmark; $H_x$, $H_c$, and $H_s$ are activity, chain, and structural HHI; $L_{\max}$ is the activity share lost with the largest route. Values are not empirical estimates.
\end{tablenotes}
\end{table}


==> release/sections/01_introduction.tex <==
\section{Introduction}\label{sec:introduction}

Decentralized finance (\DeFi{}) seeks to provide financial services through public blockchains and smart contracts rather than conventional centralized intermediaries \cite{schar2021defi,werner2022sokdefi,makarov2022cryptocurrencies}. However, visible transactions and open code do not establish that a financial system is decentralized. A protocol may attract more participants while activity becomes concentrated among a smaller set of addresses. It may operate on more blockchains while relying on one bridge, router, or messaging service. It may distribute routine activity broadly while governance or economic control remains concentrated. The relevant question is therefore not whether a protocol is decentralized in the abstract, but \emph{which dimensions are dispersed, how they change, and what evidence can support each conclusion}.

We study this problem in Aave, an open-source lending protocol in which participants supply assets and borrow against collateral through smart contracts. Aave was already operating across multiple blockchains before its protocol-native GHO stablecoin launched. The two institutional changes examined here are therefore not Aave's entry into Ethereum and Arbitrum, but GHO issuance on Ethereum and GHO's subsequent expansion to an existing Aave market on Arbitrum. Aave's Pool contracts record supplying, withdrawing, borrowing, repaying, and liquidating in a consistent event format. Those records reveal blockchain addresses and protocol roles, but they do not by themselves reveal the people or organizations controlling the addresses, the infrastructure paths supporting an action, or the effect of a protocol change.

Economics, finance, computer science, and network science each illuminate part of this distinction. Economics studies strategic interaction and concentration; finance studies liquidity, intermediation, and dependence; computer science makes execution records auditable; and network science measures position, temporal change, and resilience. We integrate these perspectives through a \emph{Protocol-Network Decentralization Analysis} framework. It represents decentralization at time $t$ as
\begin{equation}
\boldsymbol{\Delta}_t=\left(\mathcal P_t,\mathcal A_t,\mathcal S_t,\mathcal I_t\right),
\label{eq:decentralization-vector}
\end{equation}
where $\mathcal P_t$ denotes participation, $\mathcal A_t$ activity distribution, $\mathcal S_t$ network structure, and $\mathcal I_t$ infrastructure dependence. The dimensions are reported separately rather than collapsed into one score. Figure~\ref{fig:literature-landscape} shows how complementary insights from economics, finance, computer science, and network science inform these dimensions and connects each dimension to the measures implemented in the theoretical, simulation, and empirical components. Economic-actor decentralization is an additional interpretive layer: addresses are observable, whereas common control across addresses requires independent evidence.

\input{tables/tab01_dimensions}

The analysis addresses four questions aligned with the four dimensions. First, around GHO issuance on Ethereum and GHO's first cross-chain expansion to Arbitrum, how did address-level participation change? Second, did Pool-event-frequency concentration move with participation or diverge within each chain? Third, how did network structure vary across protocol roles, actions, chains, and scale adjustments? Fourth, what additional actor, infrastructure-route, and counterfactual evidence is required to evaluate economic control, infrastructure dependence, and causal effects?

We integrate network theory, theorem-consistent agent-based simulation, and longitudinal evidence. The theory explains how heterogeneous direct benefits propagate through an economic-interaction network, why aggregate growth need not make activity more evenly distributed, and why venue dispersion does not identify infrastructure resilience. The Mesa--NetworkX simulations use 40 rule-based actors to recover the analytical equilibrium and separately test network amplification, growth--concentration divergence, and route/component dependence across deterministic seeds and updating regimes. They are synthetic mechanism checks, not calibrated Aave estimates. The empirical analysis then constructs weekly networks from 118,806 Ethereum and 1,837,410 Arbitrum Aave V3 Pool events. Figure~\ref{fig:interdisciplinary-framework} shows how the case, methods, outcomes, and evidence boundary fit together.

\input{figures/fig01_interdisciplinary_framework}

The results show why the dimensions must remain separate. Excluding the week of each reserve activation, the mean weekly number of addresses with changing lending or borrowing positions rises by 91.0\% on Ethereum and 1.7\% on Arbitrum. Over the same chain-relative windows, concentration of observed Pool-event activity falls by 31.5\% on Ethereum but rises by 58.1\% on Arbitrum. On the common 2024 calendar, Arbitrum's participation gap relative to Gnosis widens while its HHI increases less; most of the comparative movement occurs on Gnosis and the fitted level and slope changes are sensitive to the anticipation exclusion. These are descriptive and comparative longitudinal estimates, not identified effects of GHO. The analysis further shows that conclusions about network structure depend on the protocol role being measured and on adjustment for network size.

The paper makes four contributions. First, conceptually, it represents decentralization as participation, activity distribution, network structure, and infrastructure dependence rather than as a unitary verdict. Second, theoretically and computationally, it builds on the established fixed-network game and validates three mechanisms with analytical-equilibrium-checked agent-based simulations: network amplification, growth--concentration divergence, and dispersion--resilience divergence. Third, methodologically, it converts Pool events into typed weekly address--role networks with explicit roles, dates, and scale adjustments. Fourth, empirically, it combines chain-specific longitudinal evidence with a reproducible Arbitrum--Gnosis DiD-style comparison, controlled interrupted-time-series estimates, dynamic comparative contrasts, and explicit identification diagnostics. Together, these contributions make multidimensional decentralization measurable without assigning stronger meaning to the data than they can support.

The broader implication is constructive. Rather than seek a single verdict on whether \DeFi{} is decentralized, researchers and practitioners can ask which dimension matters for a given financial function, what observable pattern a proposed mechanism predicts, and what evidence would justify a stronger conclusion. The remainder develops the institutional setting and research gap (Section~\ref{sec:background}), theory and simulation (Section~\ref{sec:model}), measurement (Section~\ref{sec:data}), longitudinal comparative evidence and identification boundaries (Section~\ref{sec:causal}), and implications (Section~\ref{sec:conclusion}).


==> release/sections/02_background.tex <==
\section{Institutional setting and research gap}\label{sec:background}

\subsection{Aave's multichain footprint and GHO's cross-chain expansion}\label{subsec:institutional}

Aave is an open-source, non-custodial liquidity protocol in which suppliers provide assets to smart-contract markets and borrowers obtain overcollateralized loans. Its institutional importance here lies in three interacting layers: public blockchains record settlement; protocol markets organize supplying, borrowing, repayment, and liquidation; and governance controls deployments, risk parameters, and approved infrastructure. Decentralization can therefore refer to access, activity, network position, governance, or technical dependence rather than one property of the codebase.

Aave's protocol footprint and GHO's asset footprint have different histories. Aave V3 first deployed on six networks in March 2022, with Arbitrum among the initial deployments, and reached Ethereum in January 2023 \cite{aave2026v3history,aave2026arbitrum}. Thus, the July 2024 event studied below is not Aave's arrival on Arbitrum; it is GHO's arrival in an Aave market that had already operated there for more than two years. Current official records list Aave deployments on Ethereum, Polygon, Avalanche, Arbitrum, Optimism, Base, BNB Chain, Scroll, Metis, Gnosis, ZKsync Era, Linea, Sonic, Celo, Soneium, Plasma, Fantom, and Harmony \cite{aave2026deployments}. These deployments define a broader comparative population, not a single common treatment date.

GHO extends this ecosystem vertically by adding a protocol-native, overcollateralized stablecoin. Governance approved its launch on Ethereum with the Aave V3 market and a FlashMinter as initial facilitators; GHO launched on 15 July 2023 \cite{aave2023gholaunch,aave2023stateq2}. Facilitators can mint and burn within governance-defined capacity limits, while borrower interest flows to the Aave DAO \cite{aavegho2026,aavefacilitators2026}. This design can deepen activity and attract participants, but it can also concentrate issuance capacity, liquidity, or routing. Stablecoin growth and decentralization are therefore distinct outcomes.

Cross-chain GHO extends the same asset horizontally. Ethereum remains the issuance anchor while approved facilitators and Chainlink's Cross-Chain Interoperability Protocol support canonical representations on destination chains \cite{aave2024crosschainlaunch,aavebridge2026}. Arbitrum was the first destination and GHO launched there on 2 July 2024, with bridge capacity subsequently expanded \cite{aave2024ghoarbitrumdate,aave2024arbitrumcapacity}. Cross-chain access can broaden venue choice while increasing common dependence on a limited route set. This tension motivates the distinction between chain dispersion and infrastructure resilience.

The GHO footprint continued to expand after the two events analyzed in this paper. By July 2025, GHO was available on Base, Lens, and Avalanche in addition to Ethereum and Arbitrum; by August 2025, a Gnosis market had also been deployed \cite{aave2025gholaterchains,aave2025ghognosis}. Later deployments are verified candidates for future longitudinal study, not observations in the present Ethereum--Arbitrum panels. This distinction is especially important for Gnosis: the paper's same-calendar 2024 Gnosis series is used only to test comparison suitability, whereas the later GHO deployment creates a separate prospective study cohort.

These changes provide verifiable clocks, not automatic experiments. Governance discussion, anticipated demand, market conditions, and chain-specific trends can precede implementation. We use the clocks to organize transparent longitudinal windows and reserve causal interpretation for designs with credible counterfactual support. Figure~\ref{fig:institutional-timeline} distinguishes Aave's pre-existing multichain development from the two GHO events examined here, identifies the weekly observation windows, and connects the comparisons to the four separately reported dimensions of decentralization.

\input{figures/fig02_institutional_timeline}

\subsection{What existing literatures explain---and leave disconnected}\label{subsec:literature}

Economics explains how strategic interaction and network position shape aggregate behavior. Fixed-network games characterize equilibrium amplification and key-player logic \cite{jackson1996strategic,galeotti2010network,ballester2006keyplayer,bramoulle2014strategic}; graphon games extend this logic to approximations and interventions in large heterogeneous networks \cite{parise2023graphon}. The present model retains a finite, observed network and uses the large-network literature as an extension rather than as an implemented estimator.

Finance focuses on intermediation, liquidity, concentration, and the allocation of rents. Research on lending protocols studies interest-rate and liquidity mechanisms \cite{gudgeon2020loanable}, while broader \DeFi{} research shows that open architecture can coexist with concentrated governance, operational dependencies, or new intermediaries \cite{schar2021defi,aramonte2021defi,makarov2022cryptocurrencies,jensen2021governance,werner2022sokdefi}. Recent empirical synthesis documents the growing use of transaction-level data while emphasizing persistent measurement and identification challenges \cite{leon2026data}. Recent decentralized-exchange studies further show that execution infrastructure can redirect arbitrage rents and that priority-fee bidding contains information about trader behavior \cite{capponi2025liquidity,capponi2026price}. These market-microstructure results motivate attention to infrastructure and role-specific behavior, but they do not establish corresponding effects in Aave lending markets.

Computer-science research makes protocol execution observable while exposing technical dependencies. Work on blockchain interoperability distinguishes architectures and trust assumptions \cite{belchior2021survey}; systematizations of \DeFi{} emphasize composability, smart-contract execution, and protocol risks \cite{schar2021defi,werner2022sokdefi}, while transaction-level composition research shows how nominally separate protocols become interdependent through nested financial and software relations \cite{kitzler2023disentangling}. Record linkage adds a separate warning: repeated addresses are not verified people or organizations without an evidence-based entity model \cite{binette2022entity}. Thus public execution records improve measurement without resolving common control or route dependence by themselves.

Network science supplies measures of centrality, coreness, communities, temporal change, and multilayer organization \cite{borgatti2000models,rombach2017core,kojaku2018core,holme2012temporal,kivela2014multilayer}. Recent methods distinguish nodewise from layerwise connectivity and detect core--periphery structure jointly across nodes and layers \cite{presigny2024duality,bergermann2025multilayercore}. They sharpen the future multilayer agenda, but the present study does not implement those estimators because verified interlayer route edges are unavailable. Financial-network research provides the economic complement: dependencies can support matching while transmitting shocks through central institutions \cite{elliott2014financial,acemoglu2015systemic,demange2018threat}.

Causal-inference research explains why public event dates do not identify effects by themselves. Staggered adoption, heterogeneous responses, limited comparison units, and divergent pre-trends require designs beyond simple before--after contrasts \cite{goodmanbacon2021difference,callaway2021difference,sun2021estimating,abadie2010synthetic,arkhangelsky2021synthetic}. Together, these literatures imply that the unit of analysis, network relation, timing convention, counterfactual, and scope of interpretation must be stated separately.

Figure~\ref{fig:literature-landscape} makes this integration operational by mapping the four disciplinary foundations to the four PNDA dimensions and then to the measures used in this study. Its categorical ribbons express conceptual relationships rather than literature counts or evidentiary strength. The fixed-corpus quantitative coding audit is reported separately in Appendix~\ref{app:literature-coding}; it is retained for reproducibility and is not presented as an exhaustive map of the related-work corpus.

\input{figures/fig02b_literature_landscape}

\subsection{Research gap and positioning}

The missing link is an integrated framework that moves from economic mechanism to an observable protocol network while preserving the limits of each source of evidence. The component literatures establish strategic amplification, financial intermediation, auditable execution, structural measurement, and identification requirements, but they authorize different claims from different evidence objects. This paper's contribution is therefore integrative rather than a claim to invent each component: it connects mechanism, simulation, role-aware temporal networks, scale-adjusted structure, and longitudinal evidence within one four-dimensional framework.


==> release/sections/03_model_simulation.tex <==
\section{Network theory and theorem-consistent agent-based simulation}\label{sec:model}

This section separates three evidence objects. The analytical model establishes conditional implications on a fixed economic-interaction network. The agent-based simulations test whether transparent update dynamics recover those implications and expose their adjustment paths. The longitudinal analysis in Sections~\ref{sec:data}--\ref{sec:causal} measures address-level outcomes around protocol events. Simulation is therefore a bridge from mechanism to observable questions, not a substitute for empirical evidence.

\subsection{Economic-interaction model}\label{subsec:model}

Let $N=\{1,\ldots,n\}$ be potential actors, $x_i\geq0$ actor $i$'s activity, and $G=(g_{ij})$ a nonnegative, possibly directed economic-interaction matrix. The entry $g_{ij}$ records how strongly actor $j$'s activity enters actor $i$'s incentive, so the corresponding influence edge is $j\rightarrow i$. This theoretical matrix is not automatically identical to the empirical action-side-to-position-holder network constructed from Pool events. Table~\ref{tab:model-notation} summarizes the objects used below.

\input{tables/tab_model_notation}

Under protocol condition $p$, $b_i(p)$ is actor $i$'s direct net benefit and $\beta\geq0$ is the strength of strategic complementarity. Conditional on $G$ and $p$, the canonical linear--quadratic payoff is
\begin{equation}
u_i(x_i,x_{-i};p)=b_i(p)x_i-\frac12x_i^2
+\beta x_i\sum_j g_{ij}x_j.
\label{eq:payoff-main}
\end{equation}
Accordingly,
\begin{equation}
\frac{\partial x_i}{\partial\left(\sum_jg_{ij}x_j\right)}=\beta
\label{eq:beta-interpretation}
\end{equation}
on an interior best response. Thus $\beta$ measures how strongly an actor responds to weighted activity by economically connected actors, while $G$ determines where that response can propagate. In an Aave analogy, additional liquidity from Bob changes Alice's modeled borrowing or participation little when $\beta$ is low and more strongly when $\beta$ is high; Alice's response can then affect other connected actors. The parameter is not an interest rate, probability, number of links, estimated GHO effect, or blockchain-specific constant.

Because raw $\beta$ depends on the scale of $G$, define normalized network-feedback strength as
\begin{equation}
\kappa=\beta\rho(G),
\label{eq:kappa}
\end{equation}
where $\rho(G)$ is the spectral radius. The simulations normalize $G$ so that $\rho(G)=1$, making $\kappa=\beta$. Protocol events enter as heterogeneous direct-benefit changes, $b^1=b^0+\Delta b$. GHO issuance on Ethereum can represent access, borrowing, liquidity, arbitrage, repayment, or liquidation opportunities; expansion to Arbitrum can additionally represent destination availability, lower transaction costs, integrations, liquidity, and infrastructure exposure. These analogies motivate $\Delta b_i$ but do not identify its historical value or imply that every actor benefits.

\begin{lemma}[Canonical optimal response]\label{lem:optimal-response}
For fixed $x_{-i}$, Equation~\eqref{eq:payoff-main} is strictly concave in $x_i$ and has the unique best response
\begin{equation}
x_i=\max\!\left\{0,\ b_i(p)+\beta\sum_jg_{ij}x_j\right\}.
\label{eq:best-response}
\end{equation}
On an interior active set, the stacked response system is $x=b(p)+\beta Gx$.
\end{lemma}

We use a short-run benchmark: $G$ is predetermined during a comparison, the same active set remains interior, and $\beta\rho(G)<1$. This isolates the intensive margin $x_i^0\rightarrow x_i^1$. Entry, exit, and structural change $G_0\rightarrow G_1$ remain outside the present equilibrium result. Appendix~\ref{app:formal-model} gives the full proofs, richer benefit function, and boundary cases.

\subsection{Three analytical results}\label{subsec:theory-results}

\subsubsection{Network amplification}

\begin{lemma}[Walk expansion]\label{lem:walk-expansion}
Under the maintained assumptions,
\begin{equation}
(I-\beta G)^{-1}=I+\beta G+\beta^2G^2+\cdots,
\label{eq:walk-expansion}
\end{equation}
and every term is elementwise nonnegative. The $(i,j)$ entry of $G^k$ aggregates length-$k$ directed walks from actor $j$ to actor $i$.
\end{lemma}

The equilibrium is
\begin{equation}
x^{*}(G,p)=(I-\beta G)^{-1}b(p).
\label{eq:equilibrium}
\end{equation}

\begin{theorem}[Unique equilibrium and network amplification]\label{thm:equilibrium-multiplier}
Fix $G$ and an interior active set. If $G$ is nonnegative, $b(p)>0$, and $\beta\rho(G)<1$, the game has the unique equilibrium in Equation~\eqref{eq:equilibrium}. For any scalar change $t$ with $\partial b/\partial t\geq0$,
\begin{equation}
\frac{\partial x^{*}}{\partial t}=(I-\beta G)^{-1}\frac{\partial b}{\partial t}\geq0.
\label{eq:network-multiplier-main}
\end{equation}
A direct gain can therefore increase activity among actors reached through positive-weight network paths.
\end{theorem}

\paragraph{Meaning, analogy, and boundary.}
Mathematically, the inverse multiplier propagates a direct-benefit change along weighted walks. In network terms, feedback strength and path structure jointly determine amplification. In an Aave analogy, an opportunity first available to a supplier, borrower, liquidator, or intermediary can affect connected roles as their incentives respond. A three-actor line gives the intuition: Alice responds directly, Bob responds to Alice, and Chen responds through Bob. The result does not establish that the empirical Aave network equals $G$, that links are exogenous, or that GHO caused an observed change. Existence, uniqueness, and the multiplier are inherited from canonical network games \cite{ballester2006keyplayer,bramoulle2014strategic,jackson2015games}; the paper-specific use is to connect heterogeneous protocol benefits to separately measured decentralization outcomes.

\subsubsection{Growth and concentration}

Let $X=\sum_i x_i^{*}$, $q_i=x_i^{*}/X$, and
\begin{equation}
H_x=\sum_iq_i^2.
\label{eq:activity-hhi}
\end{equation}

\begin{lemma}[How an actor's share changes]\label{lem:share-change}
Along a differentiable change $t$ that preserves the active set, let $m_i=\partial x_i^{*}/\partial t$ and $M=\sum_i m_i$. Then
\begin{equation}
\frac{\partial q_i}{\partial t}=\frac{m_i-q_iM}{X}.
\label{eq:share-change}
\end{equation}
Actor $i$ gains share precisely when its marginal gain exceeds its current share of the aggregate gain.
\end{lemma}

\begin{theorem}[Growth--concentration divergence]\label{thm:growth-concentration}
Under the conditions of Lemma~\ref{lem:share-change},
\begin{equation}
\frac{\partial H_x}{\partial t}=\frac{2}{X}\sum_i(q_i-H_x)m_i.
\label{eq:hhi-sign-main}
\end{equation}
The sign of concentration change is therefore independent of the growth condition $\partial X/\partial t=\sum_i m_i>0$.
\end{theorem}

\paragraph{Meaning, analogy, and boundary.}
Mathematically, HHI falls when marginal activity is sufficiently tilted toward actors below the concentration-weighted share benchmark, remains unchanged under proportional growth, and rises when gains favor actors already above that benchmark. In network terms, amplification says how a response spreads; the recipients determine whether shares converge or diverge. In an Aave analogy, the same aggregate expansion can reflect smaller holders catching up, all holders growing proportionally, or large incumbents pulling ahead. The theorem does not identify which allocation occurred historically, translate addresses into independent economic actors, or assign a causal mechanism to a measured HHI change.

\subsubsection{Chain dispersion and infrastructure resilience}

If removing route $k$ reduces feasible activity from $X$ to $X^{-k}$, define route-removal loss
\begin{equation}
L_k=(X-X^{-k})/X.
\label{eq:removal-loss}
\end{equation}
Let $c_v$ be the share of activity recorded on chain $v$, so chain concentration is $H_c=\sum_vc_v^2$, and let $r_k$ be the share made immediately unreachable by failure of route $k$ before behavioral substitution.

\begin{lemma}[Location shares do not identify route exposure]\label{lem:location-route}
For destination share $s>0$ and $R\geq1$ routes, any nonnegative allocation satisfying $\sum_kr_k=s$ has the same chain shares, while
\begin{equation}
\frac{s}{R}\leq\max_k r_k\leq s.
\label{eq:route-exposure-bounds}
\end{equation}
\end{lemma}

\begin{theorem}[Chain dispersion does not imply route resilience]\label{thm:dispersion-resilience}
Suppose activity initially lies on one chain and share $s\in(0,1/2]$ moves to a destination chain. Chain HHI falls by $2s(1-s)$. If all destination activity depends on one non-substitutable route, direct single-route exposure remains $s$. If that exposure is divided equally across $R$ independent, non-overlapping routes, the largest direct single-route exposure is $s/R$.
\end{theorem}

\paragraph{Meaning, analogy, and boundary.}
Mathematically, venue shares leave route allocation underidentified. In network terms, where activity appears and which dependencies keep it reachable are different layers. In the focal analogy, Ethereum and Arbitrum can have balanced activity shares while remote activity still relies on one designated interoperability stack; several nominal routes can also share one critical component. The theorem does not estimate a historical route-removal loss, establish independence among internal components, or model adaptive rerouting. It characterizes the data needed to test infrastructure resilience rather than inferring resilience from chain count.

\subsection{Dynamic agent-based validation of the theoretical mechanisms}\label{subsec:simulation}

The simulations implement Equation~\eqref{eq:best-response} with transparent rule-based agents in Mesa 3 and directed networks in NetworkX; NumPy/SciPy supplies an independent analytical benchmark \cite{terhoeven2025mesa}. They illustrate mechanisms implied by the analytical results. They are not calibrated estimates of historical Aave behavior and do not constitute causal evidence about GHO issuance or cross-chain expansion.

All experiments use 40 actors. For stable configurations, each run stops when $\lVert x^{(\ell+1)}-x^{(\ell)}\rVert_2<10^{-9}$ or at its disclosed horizon (1,500 iterations in the general protocol and 700 for Experiment 2) and is checked against Equation~\eqref{eq:equilibrium}. The primary network uses deterministic seed 20260819; robustness exercises use five seeds across sparse, core--periphery, and modular networks and simultaneous, fixed sequential, and randomized asynchronous activation. The named feedback conditions are $\kappa\in\{0,0.25,0.50,0.75,0.95\}$. The $\kappa=1.05$ assumption-violation test is reported separately and is not pooled with theorem-consistent cases. Appendix~\ref{app:simulation-protocol} provides the complete protocol, and Appendix~\ref{app:simulation-sensitivity} reports validation and sensitivity checks.

Figure~\ref{fig:three-theory-simulations} places the three matched experiments on one page. Row (a) applies equal-mass shocks to influence-central, peripheral, and broad actor sets, traces update iterations, and compares responses over directed distance at $\kappa=0.25,0.75,0.95$. Row (b) holds shock mass fixed while allocating benefits toward peripheral actors, in proportion to baseline activity, or toward incumbents; seed-level points and 5th--95th simulation intervals remain categorical. Row (c) fixes activity shares at 60\% on the issuance chain and 40\% on a synthetic destination while varying independent routes and shared components.

\input{generated/simulation/simulation_results_macros}

\begin{figure}[p]
\centering
\suspendrefereelines
\includegraphics[width=\textwidth,height=.78\textheight,keepaspectratio]{generated/simulation/figure_three_theory_simulations.pdf}
\resumerefereelines
\caption{Theorem-consistent agent-based simulations. (a) A direct benefit propagates through a directed economic-interaction network. The middle panel shows distance to equilibrium; the right panel reports mean activity response by directed distance for $\kappa=0.25,0.75,0.95$ on a logarithmic response scale, with error bars equal to plus or minus one standard error across actors at each distance. Distance zero contains the single shocked actor. Stronger stable feedback increases amplification, persistence across network distance, and convergence time. (b) Equal-mass benefit allocations make total activity grow while activity HHI falls, remains unchanged, or rises according to the recipients of marginal activity. Points show deterministic seeds and intervals span the 5th--95th percentiles. (c) Identical 60/40 chain shares imply chain HHI of 0.52 in every synthetic configuration, while worst immediate loss depends on independent routes and shared components. All structures and outcomes are synthetic and are not calibrated estimates of historical Aave behavior or deployed-route failures.}
\label{fig:three-theory-simulations}
\label{fig:simulation-outcomes}
\end{figure}

The first experiment converges in \SimIterWeak{}, \SimIterStrong{}, and \SimIterNear{} simultaneous iterations at $\kappa=0.25,0.75,0.95$; the maximum stable analytical-equilibrium error is \SimMaxAnalyticError{}. The $\kappa=1.05$ boundary test does not converge. At directed distances $0,1,2,3$, mean activity responses are $(1.015,0.0467,0.00391,0.000106)$ for $\kappa=0.25$, $(1.326,0.321,0.0980,0.00887)$ for $\kappa=0.75$, and $(3.399,1.822,0.768,0.0918)$ for $\kappa=0.95$. The logarithmic axis keeps the weak-feedback profile visible. The separation among the curves shows that stronger complementarity raises not only the direct response but also the magnitude retained after additional network steps; the error bars describe within-network heterogeneity among actors at the same distance rather than historical sampling uncertainty.

The second experiment uses ten deterministic network seeds. Median activity and HHI changes are \SimPeripheralActivity{} and \SimPeripheralHHI{} under peripheral expansion, \SimProportionalActivity{} and approximately zero under proportional growth, and \SimIncumbentActivity{} and \SimIncumbentHHI{} under incumbent amplification. These are different benefit allocations, not different values of $\beta$. In the third experiment, chain HHI remains \SimChainHHI{} while worst route loss falls from 40\% to 10\% as one route becomes four independent routes; four nominal routes sharing one critical component retain a 40\% component-loss exposure.

\input{generated/simulation/simulation_results_table}

\subsection{From mechanisms to observable evidence}

Table~\ref{tab:theory-evidence-bridge} maps each theoretical result to its simulation output and empirical counterpart. The first experiment asks whether a protocol-related benefit is followed by activity beyond its most directly exposed actors, but direct exposure and the theoretical economic links are only partially observed. The second establishes why aggregate growth is insufficient to infer decentralization: holder and action-side HHI must be reported alongside participation. The third shows why dispersion across blockchains cannot establish resilience without verified information on route independence, substitutability, and shared components.

\input{tables/tab_theory_evidence_bridge}

The empirical analysis therefore reports participation, activity distribution, structural position, and infrastructure proxies separately and treats route-level resilience as theoretically characterized but presently unmeasured. Synthetic and empirical percentage changes are not compared as if they shared units, actors, or counterfactuals. Before results are interpreted, Section~\ref{sec:causal} states all joint activity--concentration directions; theoretical labels are applied only as descriptive classifications after the measured outcomes are presented.

\FloatBarrier



==> release/sections/04_data_open_science.tex <==
\section{Measurement: from protocol events to networks}\label{sec:data}

\subsection{Observed events and analysis windows}

The unit of observation is a decoded Aave V3 Pool event. We analyze Supply, Withdraw, Borrow, Repay, and LiquidationCall events across all observed reserve assets. This choice measures how frequently addresses participate in protocol actions; it does not equate heterogeneous token quantities with a common monetary value.

Ethereum and Arbitrum are observed for event weeks $-16$ through $+16$ around verified GHO reserve activations: 15 July 2023 on Ethereum and 2 July 2024 on Arbitrum. The resulting panels contain 118,806 and 1,837,410 retained Pool events, respectively. The common-calendar analysis aligns the Arbitrum and Gnosis series to the verified Arbitrum execution time, 2 July 2024 at 15:40:32 UTC, and covers 33 complete seven-day windows from 12 March through 29 October 2024. It contains the same 1,837,410 Arbitrum events and 81,814 Gnosis events. All 33 chain-weeks are present; no weekly outcome is interpolated. Exact Pool contracts, block bounds, UTC timestamps, event interfaces, provider checks, and extraction limitations are documented in the appendices and supplementary materials.

\input{tables/tab02_data_network_definition}

Figure~\ref{fig:research-design} records the measurement sequence and the boundary between quantities observed in the present data and quantities that require additional evidence.

\input{figures/fig01_research_design_v2}

\subsection{Why protocol roles matter}

A blockchain transaction can call a router that internally reaches the Aave Pool. Treating the top-level sender and receiver as the economic relation would therefore confuse execution routing with protocol participation. We instead decode the Pool receipt log and retain its native roles. Each event identifies the address carrying out the action (the \emph{action-side address}) and the address whose lending position changes (the \emph{position-holder address}); the Pool records the event but is not automatically treated as a participant. Figure~\ref{fig:tx-log-network} illustrates the distinction.

\input{figures/fig04_tx_call_log_network}

Weekly networks preserve action type and reserve identity. For chain $c$ and week $t$, the two primary common-calendar outcomes are
\begin{align}
Y^{P}_{ct} &= \log\!\left(1+\mathrm{ActivePositionHolderAddresses}_{ct}\right),
\label{eq:empirical-participation}\\
Y^{A}_{ct} &= \mathrm{PositionHolderEventHHI}_{ct}
=\sum_i s_{ict}^{2},
\qquad
s_{ict}=\frac{n_{ict}}{\sum_j n_{jct}},
\label{eq:empirical-hhi}
\end{align}
where $n_{ict}$ is address $i$'s retained Pool-event count. The first outcome measures address-level participation breadth; the second measures the concentration of observed activity among position-holder addresses. Higher HHI indicates that fewer addresses account for more observed actions. The legacy machine-field name \texttt{beneficiary\_address} is rendered throughout the paper as \emph{position-holder address}. An address is an observable blockchain identifier rather than a verified person, institution, or independently controlled economic actor, so participation breadth does not equal a unique-user count.

Adjacent-week entrants, retained addresses, and exits reveal whether a participation stock reflects persistent use or rapid turnover. Self-directed Pool events remain in breadth and activity-HHI calculations because they are observed protocol actions. Structural measures instead use only non-self delegated or third-party role relations, and self-loops are excluded from topology because a self-directed action does not reveal delegation. Weekly aggregation uses the half-open UTC intervals documented with the data; missing calendar cells would be retained and reported rather than silently interpolated, although none occur in the 33-week common-calendar panel.

The analysis also separates role from scale. Action-side and position-holder concentration answer different economic questions. Likewise, raw PageRank HHI falls mechanically as the number of nodes increases, so cross-graph interpretation uses scale-adjusted quantities alongside coreness and persistence. Appendix~\ref{app:indicator-registry} provides the complete 39-indicator registry, formulas, units, and measurement conventions.

\subsection{Addresses, actors, and infrastructure}

An address can represent a person, exchange system, treasury, router, bridge, or contract. Address-level concentration is therefore observable, while economic-actor concentration requires verified evidence about common control. We report conservative actor-concentration bounds rather than infer ownership from behavior, timing, or bytecode similarity.

Infrastructure dependence requires another missing relation: verified links from economic activity to bridges, facilitators, messaging paths, or routes. Contract incidence alone cannot establish this mapping. Route concentration and removal-loss measures are therefore defined by the theory but reserved for a future route-event layer. This distinction is central to the framework: it identifies what would make a stronger claim possible rather than replacing missing relations with assumptions.

\subsection{Evidentiary scope}

Each reported result is tied to a stated source, observation window, network definition, and measure. Checks of event uniqueness, temporal boundaries, role semantics, and graph construction establish the domain in which a statistic is meaningful. The paper distinguishes measured outcomes from simulations, bounds, diagnostic comparisons, and quantities for which the required data are unavailable. This discipline is substantive: it determines whether an observed pattern supports an address-level description, an actor-level interpretation, a claim about infrastructure, or a causal conclusion.


==> release/sections/05_causal_inference.tex <==
\section{Longitudinal comparative evidence and identification boundaries}\label{sec:causal}

\subsection{Theory-informed interpretation before observing outcomes}\label{subsec:interpretation-framework}

The analytical and simulated mechanisms permit all joint directions in Table~\ref{tab:activity-concentration-classification}. This classification is stated before reporting the empirical estimates to avoid using observed signs to redefine a favored mechanism. ``Consistent with'' denotes a descriptive joint pattern, not proof of the behavioral process or an estimate of $\beta$.

\begin{table}[t]
\centering
\caption{Prespecified classification of joint activity and concentration changes.}
\label{tab:activity-concentration-classification}
\AVTableSetup
\begin{tabularx}{\textwidth}{P{0.21\textwidth}P{0.25\textwidth}Y}
\toprule
Activity response & Concentration response & Theory-consistent descriptive interpretation \\
\midrule
Rises & HHI falls & Peripheral expansion \\
Rises & HHI approximately unchanged & Proportional growth \\
Rises & HHI rises & Incumbent amplification \\
Falls & HHI falls & Contraction with relative equalization \\
Falls & HHI approximately unchanged & Proportional contraction \\
Falls & HHI rises & Concentrated contraction or peripheral exit \\
\bottomrule
\end{tabularx}
\end{table}

Activity and HHI alone are insufficient. A peripheral-expansion pattern would ordinarily be reinforced by broad growth in active holders, lower holder and action-side HHI, greater third-party participation, and dispersal of centrality or persistent cores. An incumbent-amplification pattern would ordinarily show the opposite tendencies, although contract-mediated and curated-infrastructure shares are theoretically ambiguous in both cases. Empirical dimensions can therefore conflict: participation may broaden while structural position concentrates, activity HHI may fall while infrastructure dependence rises, and address counts may increase without greater economic-entity diversity. We report the four dimensions separately rather than convert this classification into a composite decentralization score.

\subsection{Chain-specific participation and activity concentration diverge}

The Ethereum and Arbitrum panels contain 1,956,216 Aave V3 Pool events. Self-directed events represent 76.79\% of Ethereum events and 76.99\% of Arbitrum events; the remaining 27,579 and 422,834 events form the delegated address-role topology. Table~\ref{tab:aggregate-sample} summarizes the sample.

\input{tables/tab03_aggregate_sample}

Figure~\ref{fig:real-v5-cross-chain} provides the paper's central empirical comparison. Excluding activation week zero, mean weekly active position-holder addresses increase from 762.7 to 1,456.4 on Ethereum (91.0\%) and from 7,990.3 to 8,123.4 on Arbitrum (1.7\%). Mean weekly position-holder-event HHI falls from 0.00956 to 0.00655 on Ethereum ($-31.5\%$) but rises from 0.00932 to 0.01474 on Arbitrum ($+58.1\%$) over the same chain-relative windows. Pooling events within the pre and post periods instead yields Ethereum position-holder HHI values of 0.005647 and 0.003555, a 37.0\% decline. HHI is nonlinear, so this pooled-period statistic answers a different question from the mean weekly comparison; it is reported because the pooled address distribution is the observed input to the actor-bound analysis in Appendix~\ref{app:real-v4-partial-identification}.

\input{figures/fig05_real_v5_cross_chain}

The substantive result is not a ranking of blockchains. It is that breadth and concentration describe different aspects of decentralization and can move differently. Ethereum combines substantial address growth with declining mean HHI, a joint pattern consistent with peripheral expansion at the address level. Arbitrum combines nearly unchanged breadth with rising concentration, a mixed pattern closer to incumbent amplification than broad peripheral expansion. These labels describe the joint signs only; they do not identify the behavioral mechanism, estimate $\beta$, or establish a GHO effect. Supporting measures tell the same multidimensional story: Ethereum requires more addresses to account for 51\% of events after the focal week, while Arbitrum requires fewer. These are descriptive all-action, all-reserve patterns around different chain-specific event dates; attributing them to GHO would require action-specific panels and a credible counterfactual.

Membership flows explain how the participation stock is sustained. Figure~\ref{fig:address-state-flows} shows large entrant and exit shares on both chains, alongside modest increases in prior-week retention. A high active-address count therefore need not imply a stable participant base. For governance and market design, the distinction matters: acquisition, persistence, and concentration are separate margins.

\input{figures/fig05d_address_state_flows}

\subsection{Arbitrum--Gnosis common-calendar comparative dynamics}\label{subsec:arbitrum-gnosis-comparison}

The chain-specific panels answer how each outcome moved around its own GHO event. A separate common-calendar design asks whether Arbitrum's path around the 2 July 2024 expansion differed from contemporaneous movement on Aave's Gnosis deployment. Gnosis did not receive the focal 2024 Arbitrum expansion and therefore removes some common calendar variation, but this role does not make its path an assumed counterfactual. The analysis estimates three related objects and reports them as comparative longitudinal evidence.

First, on the 24 included weeks---clean pre weeks $-16$ to $-9$ and post weeks $+1$ to $+16$---the conventional two-chain interaction is
\begin{equation}
Y_{ct}=\alpha+\gamma\mathrm{ARB}_{c}+\lambda\mathrm{Post}_{t}
+\beta\bigl(\mathrm{ARB}_{c}\times\mathrm{Post}_{t}\bigr)+\varepsilon_{ct}.
\label{eq:did-style}
\end{equation}
The coefficient $\beta$ is algebraically the change in the Arbitrum-minus-Gnosis mean difference; its existence does not establish that the causal estimand is identified. We estimate the equivalent weekly-gap regression so serial dependence is modeled in one aggregate time series.

Second, let $G_t=Y_{\mathrm{ARB},t}-Y_{\mathrm{GNO},t}$ and $D_t=\ind\{t\geq1\}$. The controlled interrupted-time-series specification is
\begin{equation}
G_t=\theta_0+\theta_1t+\theta_2D_t+\theta_3(t-T_0)D_t+u_t,
\qquad T_0=0,
\label{eq:controlled-its}
\end{equation}
where $\theta_1$ is the clean-pre differential slope, $\theta_2$ is the fitted comparative level shift at the excluded event-week reference, and $\theta_3$ is the post-expansion differential slope change. Segmented and controlled interrupted-time-series methods motivate this separation of level and slope changes \cite{wagner2002segmented,bernal2017interrupted,bernal2018controls}. Because weeks $-8$ through 0 are omitted, $\theta_2$ is an extrapolated level difference across that interval rather than an observed week-0 discontinuity.

Third, the weekly dynamic comparative contrast is
\begin{equation}
C_k=\left(Y_{\mathrm{ARB},k}-Y_{\mathrm{GNO},k}\right)
-\overline{\left(Y_{\mathrm{ARB}}-Y_{\mathrm{GNO}}\right)}_{k=-16:-9}.
\label{eq:dynamic-comparative-contrast}
\end{equation}
These centered arithmetic gaps display timing and heterogeneity without being relabeled as event-study treatment effects.

Figure~\ref{fig:arbitrum-gnosis-comparative-dynamics} places the observed paths, the controlled-ITS fits, and the centered gaps on one page. It shows why the comparison must be interpreted in components. For log participation, Arbitrum's clean-pre-to-post change is +0.0314 while Gnosis changes by $-1.9519$, yielding a DiD-style comparative coefficient of +1.9833. For HHI, the corresponding changes are +0.00501 and +0.02343, yielding $-0.01842$: concentration rises on both chains, but less on Arbitrum. Thus the negative comparative HHI coefficient does not mean that Arbitrum concentration fell. The controlled-ITS estimates are likewise conditional on the chosen trend specification: the week-0-referenced level and slope shifts are +4.0396 and +0.1845 per week for log participation, and $-0.02849$ and $-0.003515$ per week for HHI.

\input{figures/fig07_arbitrum_gnosis_comparative_dynamics}
\input{tables/tab06_arbitrum_gnosis_main_results}
\FloatBarrier

The comparison is economically informative but specification-sensitive. Excluding no anticipation weeks reduces the participation DiD-style coefficient to +1.3414 and changes the HHI coefficient to +0.00595; four- and eight-week exclusions move both coefficients, and the controlled-ITS terms change sign under some alternatives. By contrast, the $+8$, $+12$, and $+16$ post horizons preserve the primary coefficient directions. Appendix~\ref{app:benchmark-did} reports these results, the differential pre-slopes, and placebo calculations. The pattern therefore establishes that GHO expansion coincided with a widening Arbitrum--Gnosis participation gap and a smaller relative increase in Arbitrum HHI, while also showing that Gnosis movement and differential trends are central to that comparison.

\subsection{Roles and graph scale change structural interpretation}

The full delegated graphs contain 8,891 Ethereum nodes and 50,693 Arbitrum nodes. Action-side strength is substantially more concentrated than position-holder strength on Ethereum, whereas the cross-chain pattern reverses for some measures. Figure~\ref{fig:action-layer-profile} further shows that supplying, borrowing, repaying, and liquidating generate distinct topologies. Liquidation, despite its small event share, produces the largest maximum-$k$-core share on Ethereum. These results illustrate why an aggregate network should preserve its typed layers.

\input{tables/tab05_real_v5_topology}
\input{figures/fig05b_action_layer_profile}

Graph size also changes what raw centrality concentration appears to show. After adjusting PageRank HHI for node count, the effective PageRank-node fractions are 99.41\% on Ethereum and 98.01\% on Arbitrum. Figure~\ref{fig:centrality-roles} separates this near-uniform global mass from the much smaller discrete core sets and from the protocol-decoded roles appearing in high-coreness tails. The lesson is methodological and substantive: broad global centrality can coexist with a small operational core.

\input{figures/fig05c_centrality_roles}

The fitted Borgatti--Everett cores contain two nodes on each chain, the algorithmic minimum, and are nested inside each chain's maximum-$k$ core. Public labels associate available core addresses with protocol-adjacent helper, gateway, or migration functions. This supports a narrow infrastructure-oriented interpretation of the observed address-role core, not a claim about ownership or natural persons. The 160-node backbone visualization is used for inspection; numerical conclusions come from the full graph.

\subsection{Comparison validity, uncertainty, and further causal identification}

Difference-in-differences supports causal interpretation only when the comparison path supplies the relevant counterfactual trend and anticipation, spillovers, and concurrent shocks are adequately addressed \cite{roth2023trending}. The present design improves on an Arbitrum-only before--after comparison, but the Gnosis participation path differs during the clean pre-period, its HHI series contains large weekly movements, and most of the arithmetic participation contrast is the contemporaneous Gnosis decline. Failure to reject a pre-trend test would not establish parallel trends because such tests can have low power and conditioning analysis on a pretest can distort inference \cite{roth2022pretest}. We therefore report the raw paths and differential slopes and treat sensitivity to bounded nonparallel trends as an important future extension \cite{rambachan2023credible}.

Serial correlation can materially understate uncertainty in DiD applications \cite{bertrand2004trust}. The reported Bartlett/Newey--West ranges account for modeled temporal dependence in the weekly Arbitrum-minus-Gnosis series \cite{newey1987simple}. They use fixed lags---three for the DiD-style mean-change model and two for the controlled ITS---without a finite-sample correction. With two aggregate chain series, these model-based ranges do not reproduce conventional many-cluster treatment-assignment inference. Methods for a small number of treated units still require an informative collection of untreated units and do not resolve a one-comparison-chain design \cite{conley2011inference}.

Further causal identification can build same-semantic panels for additional protocol markets, prespecify anticipation windows, validate comparison support, and use repeated GHO expansion events. Group-time, interaction-weighted, and imputation event-study methods become relevant only with multiple adoption cohorts and appropriate not-yet-treated comparisons \cite{callaway2021difference,sun2021estimating,goodmanbacon2021difference,borusyak2024revisiting}. Synthetic comparison designs likewise require a larger verified donor pool, stable pre-event fit, predictor balance, and placebo evidence. These methods define the next stage of the research program; they are not estimators silently attributed to the current two-chain analysis.

\subsection{Integrated interpretation and evidentiary boundary}

Taken together, the evidence is consistent with the framework's central distinction. Expanded access can coincide with different concentration paths; participation levels can mask substantial turnover; role definitions alter concentration; and scale adjustment changes structural comparisons. The present data establish these address-level and comparative patterns, not the behavioral mechanism or a causal effect of GHO. Economic-actor concentration change requires a common ownership partition supported by primary evidence, while route resilience requires verified route events. These boundaries identify the additional layers through which the framework can support a broader research program.


==> release/sections/06_conclusion.tex <==
\section{Discussion and conclusion}\label{sec:conclusion}

Whether decentralized finance is decentralized cannot be inferred from open code, transaction volume, address counts, or any single network statistic. The answer depends on the economic dimension at issue and on what the available evidence can establish about that dimension.

The theory and agent-based simulation yield the organizing insight: a direct benefit can propagate beyond the actors receiving it, aggregate growth can coexist with lower, unchanged, or higher concentration, and activity can become more dispersed across blockchains while dependence on a common component remains concentrated. Across stable configurations the simulation matches the analytical equilibrium to within $1.90\times10^{-8}$; equal-mass peripheral, proportional, and incumbent allocations generate the three concentration directions, while identical chain shares conceal route and shared-component losses. These synthetic results validate mechanisms, not historical Aave magnitudes. The Aave evidence shows why the distinctions matter. Excluding the week of each reserve activation, Ethereum combines a 91.0\% increase in the mean weekly number of addresses with changing lending positions and a 31.5\% decline in mean weekly Pool-event-frequency HHI. Arbitrum combines a 1.7\% increase in breadth with a 58.1\% increase in HHI. On the common 2024 calendar, GHO expansion coincides with a +1.9833 widening of the Arbitrum--Gnosis log-participation gap and a $-0.01842$ comparative HHI change, meaning HHI rises less on Arbitrum than on Gnosis. Because the participation result is mostly the Gnosis decline and the level/slope fits depend on the anticipation exclusion, these are comparative patterns rather than identified GHO effects. Role-aware and scale-adjusted analyses further show that conclusions about network structure depend on the economic relation being measured and on the treatment of network size.

The contribution crosses disciplinary boundaries without replacing the foundations of any one field. For economics and finance, the framework combines the familiar network multiplier with explicit distributional and dependency outcomes. For network science, it ties structural measures to economically defined roles and time units. For computer science and blockchain research, it shows how auditable execution records and reproducible rule-based simulations constrain economic interpretation. For governance and protocol design, it implies that assessments of adoption should report participation, activity distribution, structural position, and infrastructure dependence separately: more activity is not sufficient evidence of decentralization.

The study also has clear limits. Its longitudinal findings describe addresses and address roles; they do not estimate the causal effect of GHO. Claims about economic actors require evidence linking addresses under common control. Claims about route resilience require bridge, facilitator, and messaging-event data. Causal evaluation requires additional comparable chains or markets with stable pre-event support. These limits define the evidence boundary for the extensions below.

\subsection{Endogenous and dynamic network formation}\label{subsec:future-dynamic-network}

The fixed-network benchmark isolates short-run activity adjustment conditional on a predetermined interaction structure and locally stable active set. It does not claim that the Aave network is literally fixed. A dynamic extension would model
\[
G_{t+1}=\mathcal F(G_t,x_t,p_t,c_t),
\]
where $p_t$ denotes protocol conditions and $c_t$ chain and infrastructure conditions. When differentiable, the response can be decomposed as
\[
\frac{dx}{dp}=
\underbrace{(I-\beta G)^{-1}\frac{db}{dp}}_{\text{activity response on the existing network}}
+\underbrace{(I-\beta G)^{-1}\beta\frac{dG}{dp}x}_{\text{network-formation response}}.
\]
The first term is the present baseline; the second captures entry, exit, and rewiring. Depending on those primitives, lower destination-chain costs could attract smaller actors, preferential attachment could strengthen incumbent cores, chain-specific communities could make bridges into brokers, or common infrastructure could form a new core even as user-side concentration falls. Adaptive rerouting, hysteresis, and multiple activity--network equilibria are likewise plausible future outcomes. None is inferred from the present fixed-network experiment.

\subsection{Future research: from observable networks to systemic and agent-mediated decentralization}\label{subsec:future-systemic}

A first extension would represent the protocol as a dynamic, heterogeneous multilayer system rather than as separate temporal networks. Lending, GHO issuance and transfer, bridge, governance, and infrastructure relations would form distinct technological or institutional layers---not geographical regions---while evidence-supported entities connect across chains and functions. Memory-aware community detection could reveal persistent cores and longitudinal role transitions \cite{clemente2024memory}; higher-order representations could preserve events jointly involving users, contracts, assets, facilitators, and bridges \cite{iacopini2024temporal,zhang2023higherorder}; and chronology compression could select temporal resolution according to its effect on modeled dynamics rather than an arbitrary snapshot interval \cite{allen2024compressing}. Combined with uncertainty-aware entity resolution, these methods could test whether apparent participation growth reflects broader economic control.

A second extension would use counterfactual removal and cascading-failure simulations to examine whether liquidity and participation remain resilient when a bridge, facilitator, oracle, sequencer, or major liquidity provider fails. Multilayer models with higher-order couplings provide a foundation for studying how dependencies propagate across processes operating at different timescales \cite{nicoletti2024information}. This agenda moves from measuring observed decentralization to explaining cross-layer evolution, stress-testing common dependencies, and evaluating systemic decentralization. It does not convert the present route illustration into an empirical resilience estimate.

Agentic artificial intelligence creates both a methodological opportunity and a new economic-actor problem. As a method, language-model agents could supplement---not replace---the current mathematical model and rule-based simulation by representing heterogeneous suppliers, borrowers, liquidators, arbitrageurs, and governance participants with memory, bounded reasoning, adaptive strategies, and differentiated access to information and tools. EconAgent illustrates how language-model agents can enrich conventional economic agent-based models with heterogeneous decisions and multi-period adaptation \cite{li2024econagent}; validation against observed behavior would remain essential.

More fundamentally, autonomous agents may themselves become DeFi participants. The observable address may then sit within a longer provenance path:
\[
\begin{aligned}
\text{principal}&\rightarrow\text{decision agent}\rightarrow\text{wallet or contract}\\
&\rightarrow\text{protocol action}\rightarrow\text{beneficiary}.
\end{aligned}
\]
One principal may operate many agent-controlled wallets, while many users may delegate to the same model, strategy, wallet infrastructure, or service provider. Address-level participation could therefore expand while effective decision-making becomes more concentrated. Early exploratory research documents trading, portfolio, governance, and execution roles among crypto-related agents \cite{ante2025autonomous}, but it does not establish their prevalence in the Aave records studied here.

The measured decentralization vector consequently remains
\[
\boldsymbol{\Delta}_t=(\mathcal P_t,\mathcal A_t,\mathcal S_t,\mathcal I_t).
\]
A future framework could add a fifth, separately evidenced dimension,
\[
\boldsymbol{\Delta}_t^{+}=(\mathcal P_t,\mathcal A_t,\mathcal S_t,\mathcal I_t,\mathcal D_t),
\]
where \(\mathcal D_t\) denotes agency-and-delegation concentration: the concentration of effective decision-making among principals, autonomous agents, models, strategies, and service providers that initiate or coordinate on-chain activity. Candidate indicators include provider or strategy HHI, principal concentration across agent-operated wallets, shared-dependency concentration, action synchronization, and the share of autonomous versus human-confirmed execution. These quantities cannot generally be inferred from Pool events alone. They require verified agent labels, delegation and authorization records, smart-wallet permissions, intent attestations, auditable execution traces, and independently validated off-chain evidence. Appendix~\ref{app:future-systemic} provides the staged roadmap and evidence requirements.

The durable contribution is a multidimensional account of decentralization that links economic mechanism to observable network evidence. It makes previously conflated questions measurable, explains why distinct forms of decentralization can diverge, and provides a disciplined basis for studying how protocol growth, activity distribution, network structure, infrastructure dependence, and---once independently evidenced---delegated agency evolve together.


==> release/tables/tab01_dimensions.tex <==
\begin{table}[!b]
\caption{Four dimensions of effective decentralization and their evidence status.}
\label{tab:dimensions}
\centering
\AVTableSetup
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.30}
\begin{tabularx}{\textwidth}{@{}P{24mm}P{28mm}P{32mm}Y@{}}
\toprule
\AVTableHeader
\textbf{Dimension} & \textbf{Indicators} & \textbf{Interpretive question} & \textbf{Evidence in this study} \\
\midrule
\AVInlineIcon[AVBlue]{users}\textbf{Participation} & Active addresses; entry, exit, and retention & How broadly is access and continued use distributed? & \AVObservedTag\ Address-level breadth. \AVBoundedTag\ People and firms are not identified. \\
\addlinespace[1.5pt]
\AVInlineIcon[AVViolet]{chart}\textbf{Activity distribution} & Event shares; HHI; top-address shares & How evenly is observed protocol activity shared? & \AVObservedTag\ Address-level event frequency. \AVUnavailableTag\ Causal effect is not identified. \\
\addlinespace[1.5pt]
\AVInlineIcon[AVOrange]{network}\textbf{Network structure} & Role-specific connections; centrality; core membership & Which addresses occupy central or persistent positions? & \AVObservedTag\ Address-role networks. \AVBoundedTag\ Economic control is not inferred. \\
\addlinespace[1.5pt]
\AVInlineIcon[AVTeal]{bridge}\textbf{Infrastructure dependence} & Route shares; bridge or facilitator reliance; loss after route failure & Can activity continue if a common service becomes unavailable? & \AVDiagnosticTag\ Protocol-adjacent addresses. \AVUnavailableTag\ Verified route events and failure losses. \\
\bottomrule
\end{tabularx}
\begin{tablenotes}[flushleft]
\AVTableNoteFont
\item \emph{Notes:} The four dimensions are reported separately. Addresses are observable protocol identifiers, not verified people or firms. Any secondary composite index must retain transparent components, directions, and weights.
\end{tablenotes}
\end{table}



==> release/tables/tab01_general_paradigm.tex <==
\begin{table*}[t]
\centering
\caption{General protocol-network decentralization analysis paradigm.}
\label{tab:general-paradigm}
\AVTableSetup
\begin{tabularx}{0.98\textwidth}{>{\centering\arraybackslash}p{1.05cm}P{0.17\textwidth}YP{0.25\textwidth}}
\toprule
\AVTableHeader
\multicolumn{2}{l}{\textbf{Stage}} & \textbf{Research object} & \textbf{Fail-closed requirement} \\
\midrule
\AVTableIcon[AVBlue]{blocks} & \textbf{Protocol scope} & Verified contracts, chains, roles, and policy clocks & Executed and observed event, not announcement alone \\
\AVTableIcon[AVBlue]{database} & \textbf{Native events} & ABI-decoded Pool logs with block, transaction, and log keys & Emitter, signature, indexed fields, and coverage agree \\
\AVTableIcon[AVViolet]{network} & \textbf{Role network} & Typed action-side $\rightarrow$ position-holder edges by week, action, reserve, and chain & Pool emitter is not silently promoted to an economic node \\
\AVTableIcon[AVTeal]{chart} & \textbf{Evidence dimensions} & Address participation, Pool-event-frequency concentration, structural influence, and infrastructure-core or route dependence & Each dimension is classified as observed, bounded, diagnostic, simulated, rejected, or unavailable \\
\AVTableIcon[AVTeal]{clock} & \textbf{Longitudinal evidence} & Symmetric panels, topology, core--periphery, and address-to-actor bounds & Descriptive change remains distinct from an identified effect \\
\AVTableIcon[AVOrange]{filter} & \textbf{Comparative design} & Common-calendar comparison series, exclusion window, and diagnostics & Pre-paths, support, and inference determine the permitted interpretation \\
\AVTableIcon[AVViolet]{code} & \textbf{Open science} & Documented inputs, analysis programs, validation checks, and evidence table & Unsupported entity, infrastructure, or causal claims are identified explicitly \\
\bottomrule
\end{tabularx}
\end{table*}


==> release/tables/tab02_data_network_definition.tex <==
\begin{table*}[t]
\centering
\caption{Protocol-event and network construction rules.}
\label{tab:data-network-definition}
\AVTableSetup
\begin{tabularx}{0.98\textwidth}{>{\centering\arraybackslash}p{1.05cm}P{0.18\textwidth}YP{0.27\textwidth}}
\toprule
\AVTableHeader
\multicolumn{2}{l}{\textbf{Object}} & \textbf{Operational definition} & \textbf{Interpretation boundary} \\
\midrule
\AVTableIcon[AVBlue]{document} & \textbf{Observation} & Canonical Aave V3 Pool \texttt{Supply}, \texttt{Withdraw}, \texttt{Borrow}, \texttt{Repay}, or \texttt{LiquidationCall} log & Not an arbitrary top-level transaction \\
\AVTableIcon[AVViolet]{users} & \textbf{Action side} & Protocol-native caller or actor field for the action family & May be an EOA, router, adapter, or contract \\
\AVTableIcon[AVTeal]{users} & \textbf{Position holder} & \texttt{onBehalfOf} for Supply/Borrow; \texttt{user} for Withdraw/Repay/LiquidationCall & An observed address, not a verified person or institution \\
\AVTableIcon[AVTeal]{network} & \textbf{Edge} & Directed action-side $\rightarrow$ position-holder pair, weighted by event count & Pool is the verified log emitter, not automatically a node \\
\AVTableIcon[AVBlue]{clock} & \textbf{Time} & UTC event week relative to the verified activation date & Week 0 is separated from clean pre and post windows \\
\AVTableIcon[AVViolet]{chart} & \textbf{Aggregate panel} & All five actions and all reserves; action and reserve labels retained & Heterogeneous raw token amounts are never summed as value \\
\AVTableIcon[AVTeal]{network} & \textbf{Network-structure graph} & Non-self delegated/third-party address-role projection & Self-directed events stay in breadth/HHI but not topology \\
\AVTableIcon[AVOrange]{filter} & \textbf{Actor layer} & Primary-source must-links plus assumption-indexed bounds & Bytecode or behavioral similarity does not prove ownership \\
\AVTableIcon[AVOrange]{bridge} & \textbf{Infrastructure layer} & Verified route-event and dependency records & Not yet measurable; contract mediation is only a proxy \\
\bottomrule
\end{tabularx}
\end{table*}



==> release/tables/tab02_policy_mechanisms.tex <==
\begin{table}[t]
\caption{Institutional innovations, countervailing mechanisms, and empirical treatment rules.}
\label{tab:policy-mechanisms}
\centering
\AVTableSetup
\begin{tabularx}{\textwidth}{p{2.55cm}XX}
\toprule
\AVTableHeader
\textbf{Institutional change} & \textbf{Countervailing mechanism} & \textbf{Empirical object and evidence status} \\
\midrule
Historical \AAVE{} network & \textit{Gain:} transferable tokens and exchange access support circulation. \textit{Risk:} exchange deposit systems and specialized contracts become persistent hubs. & Ethereum transfer graph from the October 2020 migration; historical benchmark rather than a new treatment. \\
Native \GHO{} issuance & \textit{Gain:} lower payment and borrowing frictions. \textit{Risk:} facilitator approval, bucket capacity, collateral rules, and peg support concentrate control. & Ethereum reserve activation defines the study date; technical launch, first mint, and publicity remain separate records. \\
Cross-chain \GHO{} access & \textit{Gain:} lower-cost venues attract users and disperse activity. \textit{Risk:} bridges, messaging, and rate limits can create common-mode exposure. & Arbitrum reserve activation defines the study date. Technical readiness and indexed cross-chain occurrences remain validation records, not substitute treatment dates. \\
Capacity or incentive change & \textit{Gain:} a higher bucket or incentive relaxes a binding adoption constraint. \textit{Risk:} marginal activity is directed to one facilitator, pool, or route. & Event-intensity treatment; announcement, authorization, execution, and economically binding dates remain distinct. \\
Aave v4 Hub-and-Spoke & \textit{Gain:} shared liquidity improves capital efficiency. \textit{Risk:} hub accounting, credit lines, and emergency controls raise common-infrastructure importance. & External-validity case unless activation falls inside the predefined sample; never pooled silently with V3. \\
\bottomrule
\end{tabularx}
\begin{tablenotes}\footnotesize
\item \emph{Notes:} The table states mechanisms and pre-analysis timing rules, not estimated effects. A governance proposal identifies a candidate event but does not establish treatment; route-level claims require a verified route-event table.
\end{tablenotes}
\end{table}



==> release/tables/tab03_aggregate_sample.tex <==
\begin{table*}[t]
\centering
\caption{Audited longitudinal and benchmark samples.}
\label{tab:aggregate-sample}
\AVTableSetup
\begin{tabularx}{0.98\textwidth}{P{0.16\textwidth}Y Y Y}
\toprule
\AVTableHeader
\textbf{Audit item} & \textbf{Ethereum} & \textbf{Arbitrum} & \textbf{Gnosis comparison} \\
\midrule
Calendar role & Chain-relative panel & Focal/common calendar & Contemporaneous comparison series \\
Reference clock & 15 Jul 2023 & 2 Jul 2024 & 2 Jul 2024 \\
Event weeks & $-16{:}+16$ & $-16{:}+16$ & $-16{:}+16$ \\
Aave V3 Pool events & 118,806 & 1,837,410 & 81,814 \\
Transactions & 103,171 & --- & 78,353 \\
Position-holder addresses & 15,351 & --- & 26,020 \\
Delegated topology events & 27,579 & 422,834 & not estimated \\
Provider cross-check & pass & pass & pass \\
Permitted main use & descriptive & descriptive + comparative longitudinal analysis & comparative longitudinal analysis \\
Causal effect produced & no & no & no \\
\bottomrule
\end{tabularx}
\begin{minipage}{0.96\textwidth}
\AVTableNoteFont\emph{Notes:} Data documentation, not an empirical result. Dashes denote quantities not used as reported headline statistics in the analysis dataset, not assumed zeros. Gnosis is aligned to Arbitrum's verified activation date; its own GHO activation occurred in 2025. The series removes some common calendar variation but is not assumed to supply the counterfactual path needed for a definitive causal interpretation. All units are addresses or address roles, not verified economic actors.
\end{minipage}
\end{table*}


==> release/tables/tab03_literature_map.tex <==
\begin{table*}[t]
\caption{Literature map and the study's incremental contribution.}
\label{tab:literature-map}
\centering
\AVTableSetup
\setlength{\tabcolsep}{3.4pt}
\begin{tabularx}{0.98\textwidth}{>{\centering\arraybackslash}p{0.66cm}P{3.05cm}P{4.15cm}Y}
\toprule
\AVTableHeader
\multicolumn{2}{l}{\textbf{Literature stream}} & \textbf{Established insight and remaining gap} & \textbf{Role in this study} \\
\midrule
\AVTableIcon[AVBlue]{blocks} & \textbf{DeFi adoption} & Network effects can accelerate adoption, while open smart-contract finance can still concentrate activity and governance. & Separates adoption from participation, transaction, structural, and infrastructure decentralization. \\
\AVTableIcon[AVViolet]{network} & \textbf{Financial-network structure} & Centrality, communities, and core--periphery structure reveal intermediation; static address graphs obscure persistence, control, and graph-scale effects. & Adds temporal role measurement, actor bounds, scale diagnostics, and explicit requirements for route-level conclusions. \\
\AVTableIcon[AVBlue]{users} & \textbf{Network games} & Complementarities can amplify heterogeneous activity responses; formation and calibration require additional evidence. & Uses a stylized fixed-network activity model as organizing intuition, not as an estimated formation mechanism. \\
\AVTableIcon[AVOrange]{bridge} & \textbf{Stablecoins and interoperability} & Stability and reach depend on collateral, liquidity, governance, bridges, messaging, and route redundancy. & Uses verified institutional clocks for measurement windows while withholding GHO-specific and route-level effects. \\
\AVTableIcon[AVViolet]{filter} & \textbf{Causal inference} & Modern difference-in-differences and synthetic controls clarify counterfactuals; event narratives alone do not. & Uses a common-calendar comparison to expose how pre-trends, support, anticipation, and inference constrain policy language. \\
\AVTableIcon[AVTeal]{code} & \textbf{Open computational research} & Public ledgers do not by themselves reproduce deployments, labels, timing choices, or algorithms. & Links source records, documented data, analysis programs, claims, and editable paper figures through transparent supplementary materials. \\
\bottomrule
\end{tabularx}
\end{table*}


==> release/tables/tab04_model_predictions.tex <==
\begin{table}[t]
\caption{Model implications, observable tests, and current validation status.}
\label{tab:model-predictions}
\centering
\AVTableSetup
\begin{tabularx}{\textwidth}{P{2.35cm}P{3.55cm}P{4.0cm}Y}
\toprule
\AVTableHeader
\textbf{Mechanism} & \textbf{Model implication} & \textbf{Observable test} & \textbf{Status} \\
\midrule
Network multiplier & A benefit shock propagates along walks in $G$; multiplier-central nodes respond more strongly. & Compare event responses by pre-policy centrality and persistent coreness. & Mechanism simulated; heterogeneity test planned. \\
Distributional incidence & Total activity can rise while $H_x$ rises or falls, depending on who receives marginal gains. & Estimate breadth and concentration jointly, by pre-treatment share and role. & Descriptive directions observed; causal effect pending. \\
Cross-chain divergence & Chain HHI can fall while dependence on a common route rises. & Report chain dispersion with route HHI and targeted-removal loss. & Chain-relative outcomes observed; route layer unavailable. \\
Route redundancy & Dividing exposure across independent routes lowers maximum single-route loss. & Compare verified route redundancy and stress removal under alternative definitions. & Simulation result only; empirical route table unavailable. \\
\bottomrule
\end{tabularx}
\begin{tablenotes}\AVTableNoteFont
\item \emph{Notes:} “Observed” denotes descriptive address-level evidence, not a causal or entity-level result. Proposed and unavailable analyses remain outside the paper's current claim set.
\end{tablenotes}
\end{table}



==> release/tables/tab05_real_v5_topology.tex <==
% Generated by scripts/render_scale_adjusted_topology_table.py; do not edit.
\begin{table}[htbp]
\centering
\caption{Audited full-window address-role topology with scale diagnostics.}
\label{tab:real-v5-topology}
\AVTableSetup
\begin{tabularx}{0.94\linewidth}{Yrr}
\toprule
\AVTableHeader
\textbf{Measure} & \textbf{Ethereum} & \textbf{Arbitrum} \\
\midrule
\AVTableSubheader
\multicolumn{3}{l}{\emph{Scale and role assignment}} \\
Pool events & 118,806 & 1,837,410 \\
Delegated or third-party events & 27,579 & 422,834 \\
Role-network nodes & 8,891 & 50,693 \\
Unique directed edges & 10,896 & 69,584 \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{3}{l}{\emph{Role-weight and scale-aware diagnostics}} \\
Raw action-side strength HHI & 0.4237 & 0.1668 \\
Raw position-holder-side strength HHI & 0.0008 & 0.0067 \\
Raw PageRank HHI & 0.000113 & 0.000020 \\
PageRank HHI $\times$ node count & 1.0059 & 1.0203 \\
Effective PageRank-node fraction & 99.41\% & 98.01\% \\
Maximum $k$-core share & 0.157\% & 0.209\% \\
Persistent maximum-core share & 2.294\% & 0.152\% \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{3}{l}{\emph{Core-definition diagnostics}} \\
BE binary-core nodes (minimum allowed) & 2 & 2 \\
BE nodes contained in maximum-$k$ core & 100\% & 100\% \\
Rombach--$k$-core Spearman $\rho$ & 0.521 & 0.578 \\
\bottomrule
\end{tabularx}
\begin{tablenotes}[flushleft]
\AVTableNoteFont
\item \emph{Notes:} A directed edge runs from action-side to position-holder address and is weighted by Pool-event count. Self-directed events are excluded from topology. PageRank HHI has lower bound $1/n$; multiplying by $n$ gives 1 under a uniform distribution, and its reciprocal is the effective-node fraction. The two-node Borgatti--Everett (BE) solutions hit the algorithm's imposed minimum and are fully contained in the maximum-$k$ cores, so unequal-set Jaccard values are not interpreted as membership disagreement. The BE nodes are interpreted only as an address-role infrastructure-core diagnostic; Appendix~\ref{app:be-core-infrastructure} lists their address evidence and labeling limits. Raw graph size and density differ; no scalar cross-chain structural ranking is claimed.
\end{tablenotes}
\end{table}



==> release/tables/tab06_arbitrum_gnosis_main_results.tex <==
\begin{table*}[t]
\centering
\caption{Arbitrum--Gnosis comparative longitudinal estimates.}
\label{tab:arbitrum-gnosis-main-results}
\AVTableSetup
\begin{tabularx}{0.99\textwidth}{P{0.22\textwidth}*{5}{>{\centering\arraybackslash}X}}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Arbitrum change} & \textbf{Gnosis change} & \textbf{DiD-style change} & \textbf{cITS level shift} & \textbf{cITS slope shift} \\
\midrule
Log participation & +0.0314 & $-1.9519$ & \textbf{+1.9833}\newline (0.1916) & \textbf{+4.0396}\newline (0.4190) & \textbf{+0.1845}\newline (0.0302) \\
Position-holder-event HHI & +0.00501 & +0.02343 & \textbf{$-0.01842$}\newline (0.00540) & \textbf{$-0.02849$}\newline (0.01267) & \textbf{$-0.003515$}\newline (0.001078) \\
\bottomrule
\end{tabularx}
\begin{minipage}{0.97\textwidth}
\AVTableNoteFont\emph{Notes:} Direct empirical output. Log participation is $\log(1+\text{active position-holder addresses})$. Changes compare the clean pre-period (weeks $-16$ to $-9$) with the post-period (weeks $+1$ to $+16$); weeks $-8$ to $-1$ and week 0 are excluded. Parentheses contain Bartlett/Newey--West HAC standard errors without a finite-sample correction: lag 3 for the DiD-style mean-change coefficient and lag 2 for the controlled interrupted-time-series (cITS) coefficients. Each regression uses 24 weekly Arbitrum-minus-Gnosis gaps. The cITS level coefficient is referenced to excluded week 0. These standard errors describe modeled serial dependence in the realized aggregate gap series; they do not provide many-cluster treatment-assignment inference.
\end{minipage}
\end{table*}


==> release/tables/tab06_pilot_did.tex <==
% Generated by scripts/run_real_v5_pilot_did.py; do not edit by hand.
\begin{table}[htbp]
\centering
\caption{Two-chain event-aligned difference-in-changes pilot (diagnostic, not causal).}
\label{tab:pilot-did}
\AVTableSetup
\setlength{\tabcolsep}{2.6pt}
\begin{tabularx}{\linewidth}{Yrrrr}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Ethereum} & \textbf{Arbitrum} &
\textbf{Arb. $-$ Eth.} & \textbf{NW(4) interval} \\
\midrule
\shortstack[l]{$\log(1+N_t^{p})$\\position-holder addresses} & +0.653 & +0.002 & -0.651 & [-1.002, -0.299] \\
\shortstack[l]{Position-holder\\event HHI} & -0.00301 & +0.00542 & +0.00843 & [+0.00339, +0.01347] \\
\bottomrule
\end{tabularx}
\begin{tablenotes}[flushleft]
\AVTableNoteFont
\item \emph{Notes:} For the first outcome, $N_t^{p}$ is the number of
active position-holder addresses. Entries compare mean outcome changes from event weeks $-16$ to $-1$
and $+1$ to $+16$, omitting week zero. Each chain is aligned to its own activation in a
different calendar period, and both chains receive different protocol shocks. The
interaction is Arbitrum minus Ethereum. Newey--West lag-4 intervals describe serial
variation in the paired event-week gap only; with two treated units they do not provide
valid chain-cluster causal inference. No entry is a treatment effect.
\end{tablenotes}
\end{table}



==> release/tables/tab07_arbitrum_gnosis_benchmark.tex <==
% Values reproduced by scripts/generate_arbitrum_gnosis_comparison.py.
\begin{table*}[t]
\centering
\caption{Arbitrum--Gnosis DiD-style comparative change and model-based uncertainty.}
\label{tab:arbitrum-gnosis-benchmark}
\AVTableSetup
\begin{tabularx}{0.99\textwidth}{>{\raggedright\arraybackslash}X*{4}{>{\centering\arraybackslash}X}}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Arbitrum change} & \textbf{Gnosis change} & \textbf{DiD-style change} & \textbf{Descriptive HAC range} \\
\midrule
Log participation & +0.0314 & -1.9519 & \textbf{+1.9833} & [1.6077, 2.3589] \\
Position-holder-event HHI & +0.00501 & +0.02343 & \textbf{-0.01842} & [-0.02900, -0.00784] \\
\bottomrule
\end{tabularx}
\begin{minipage}{0.97\textwidth}
\AVTableNoteFont\emph{Notes:} Direct empirical output. The clean pre-period is weeks $-16$ to $-9$; weeks $-8$ to $-1$ and week 0 are excluded; the post-period is weeks $+1$ to $+16$. The last column is a normal approximation based on Bartlett/Newey--West HAC standard errors with lag 3 and no finite-sample correction. It describes modeled serial dependence in the aggregate weekly gap; it is not a confidence interval for a treatment effect. Position holders are protocol-observed addresses, not verified economic actors. The negative HHI contrast means that HHI rose less on Arbitrum than on Gnosis; it does not mean that Arbitrum HHI fell in absolute terms.
\end{minipage}
\end{table*}


==> release/tables/tab07_network_measure_glossary.tex <==
% Generated by scripts/render_network_measure_glossary.py; do not edit by hand.
\begin{landscape}
\suspendrefereelines
\begingroup
\setstretch{1}
\AVTableSetup
\setlength{\tabcolsep}{3pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\renewcommand{\arraystretch}{1.12}
\begin{longtable}{>{\raggedright\arraybackslash}p{3.0cm}>{\raggedright\arraybackslash}p{4.5cm}>{\raggedright\arraybackslash}p{7.1cm}>{\raggedright\arraybackslash}p{5.0cm}>{\centering\arraybackslash}p{1.3cm}}
\caption{Network-measure glossary: formulas, interpretation, evidence, and visualization coverage.}
\label{tab:network-measure-glossary}\\
\toprule
\AVTableHeader
\textbf{Indicator} & \textbf{Formula} & \textbf{Definition and direction} & \textbf{Evidence, data, and visual} & \textbf{Ref.} \\
\midrule
\endfirsthead
\multicolumn{5}{c}{\tablename\ \thetable\ (continued)}\\
\toprule
\AVTableHeader
\textbf{Indicator} & \textbf{Formula} & \textbf{Definition and direction} & \textbf{Evidence, data, and visual} & \textbf{Ref.} \\
\midrule
\endhead
\midrule
\multicolumn{5}{r}{Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Participation decentralization}} \\
\textbf{Active observed participants}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: num\_nodes (when the node set is a period's active addresses)}} & $N_t=|V_t|$ & Number of distinct observed beneficiary addresses active in period t; not a count of people or independent economic actors. \emph{Direction:} Higher means broader observed participation, conditional on the address caveat. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-cross-chain} & \cite{newman2018networks} \\
\textbf{Entrants}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: new nodes}} & $E_t=|V_t\setminus V_{t-1}|$ & Addresses active in period t but not in t-1. \emph{Direction:} Higher means more observed address entry; it need not mean new economic actors. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address}} & \AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows} & \cite{holme2012temporal} \\
\textbf{Exits}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: departing nodes}} & $X_t^{exit}=|V_{t-1}\setminus V_t|$ & Addresses active in t-1 but absent in t. \emph{Direction:} Higher means more observed address exit. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address}} & \AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows} & \cite{holme2012temporal} \\
\textbf{Retained participants and retention rate}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: retained nodes}} & $R_t=|V_t\cap V_{t-1}|;\quad r_t=R_t/|V_{t-1}|$ & Addresses appearing in two adjacent periods and their share of the prior-period set. \emph{Direction:} Higher r\_t means greater address persistence, not necessarily actor persistence. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address / share}} & \AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows} & \cite{holme2012temporal} \\
\textbf{Effective number of participants}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: inverse HHI}} & $N_{eff}=1/H;\quad H=\sum_i s_i^2$ & Number of equal-share participants that would generate the observed concentration. \emph{Direction:} Higher means a more even activity distribution. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: effective address count}} & \AVObservedTag; empirical output; derived; no standalone visual & \cite{hirschman1964paternity} \\
\textbf{Cross-chain address-set overlap}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Jaccard overlap}} & $J_t=|V_{E,t}\cap V_{A,t}|/|V_{E,t}\cup V_{A,t}|$ & Overlap of Ethereum and Arbitrum beneficiary-address sets at the same chain-relative event week. \emph{Direction:} Higher means more repeated addresses across panels; because calendar dates differ it is not contemporaneous migration. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{jaccard1901distribution} \\
\textbf{Multilayer participation coefficient}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: cross-layer participation}} & $P_i=1-\sum_{\ell}(k_{i\ell}/k_i)^2$ & Dispersion of node i's connections across network layers. \emph{Direction:} Higher means connections are spread across more layers. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score in [0,1]}} & \AVUnavailableTag; no reported output; no standalone visual & \cite{kivela2014multilayer} \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Transaction decentralization}} \\
\textbf{Total observed activity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: total\_value / event\_count}} & $X_t=\sum_i x_{it}$ & Total action count in the empirical panels or equilibrium activity in the simulation; heterogeneous token amounts are not summed across reserves. \emph{Direction:} Scale measure, not a decentralization score by itself. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: events or model activity}} & \AVObservedTag; empirical output; Fig.~\ref{fig:simulation-outcomes} & \cite{newman2018networks} \\
\textbf{Activity Herfindahl--Hirschman index}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: activity\_hhi}} & $H_t=\sum_i s_{it}^2;\quad s_{it}=x_{it}/\sum_jx_{jt}$ & Squared-share concentration of actions assigned to the stated observed unit. \emph{Direction:} Higher means greater concentration; address HHI is not actor HHI. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index in [1/n,1]}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-cross-chain}, Fig.~\ref{fig:real-v4-partial-identification} & \cite{hirschman1964paternity} \\
\textbf{Economic-actor HHI identified set}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: entity-adjusted HHI}} & $H_A\leq H_G\leq1;\quad \Delta H_G\in[H_{post}-1,1-H_{pre}]$ & Bounds actor-level concentration over all partitions allowed by the stated controller assumptions. \emph{Direction:} A set crossing zero does not identify the direction of the change. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: identified interval}} & \AVBoundedTag; partial-identification output; Fig.~\ref{fig:real-v4-partial-identification} & \cite{molinari2020partial,binette2022entity} \\
\textbf{Normalized Shannon entropy}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: entropy}} & $S_t=-\sum_i s_{it}\log s_{it}/\log n_t$ & Evenness of the activity-share distribution. \emph{Direction:} Higher means more even activity. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index in [0,1]}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{shannon1948theory} \\
\textbf{Gini coefficient}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: activity\_gini}} & $G_t=\frac{\sum_i\sum_j|x_{it}-x_{jt}|}{2n_t\sum_i x_{it}}$ & Mean pairwise inequality in observed activity. \emph{Direction:} Higher means greater inequality. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index in [0,1]}} & \AVObservedTag; empirical output; no standalone visual & \cite{gini1912variabilita} \\
\textbf{Top-p activity share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: top1pct\_share / top10pct\_share}} & $T_{p,t}=\sum_{j=1}^{\lceil pn_t\rceil}s_{(j)t}$ & Share held by the largest p fraction of observed units; p is 1\% or 10\% in the analysis panel. \emph{Direction:} Higher means greater top-tail concentration. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{newman2018networks} \\
\textbf{Minimum 51\% coalition}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: nakamoto\_51}} & $K_{.51,t}=\min\{k:\sum_{j=1}^{k}s_{(j)t}\geq0.51\}$ & Smallest number of observed units whose ordered activity shares reach 51\%. \emph{Direction:} Higher means control of the measured activity is spread across more units. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: address count}} & \AVObservedTag; empirical output; no standalone visual & \cite{zhang2022sokdecentralization} \\
\textbf{Chain concentration}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: chain\_hhi}} & $H_{chain}=\sum_{\ell}s_{\ell}^{2}$ & Concentration of activity across chain layers. \emph{Direction:} Higher means activity is concentrated on fewer chains. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index}} & \AVSimulatedTag; simulated data; Fig.~\ref{fig:simulation-outcomes} & \cite{kivela2014multilayer} \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Structural decentralization}} \\
\textbf{Graph nodes and edges}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: num\_nodes / num\_edges}} & $n=|V|;\quad m=|E|$ & Size of the address-role graph and number of unique observed ties. \emph{Direction:} Scale measures; neither alone ranks decentralization. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: nodes / edges}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{newman2018networks} \\
\textbf{Graph density}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Relative degree}} & $D=m/[n(n-1)]\ \text{(directed)};\quad D=2m/[n(n-1)]\ \text{(undirected)}$ & Fraction of possible ties that are observed under the declared graph direction. \emph{Direction:} Direction is context-dependent; density normally falls mechanically as sparse graphs grow. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{newman2018networks} \\
\textbf{Weak components and giant-component share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Components\_cnt / giant\_com\_ratio}} & $C=|\operatorname{comp}(G)|;\quad g=|V_{max}|/n$ & Number of disconnected weak components and the fraction of nodes in the largest one. \emph{Direction:} Larger g means greater reachability; it is not necessarily greater decentralization. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: count / share}} & \AVObservedTag; giant share reported; no standalone visual & \cite{newman2018networks} \\
\textbf{Directed reciprocity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: directed\_reciprocity}} & $r=m_{\leftrightarrow}/m$ & Fraction of directed edges that participate in a reciprocated dyad. \emph{Direction:} Higher means more bidirectional address-role interaction; economic meaning depends on edge semantics. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{garlaschelli2004reciprocity} \\
\textbf{Degree moments and top-hub ratio}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Degree mean / Degree std / Top10Degree mean / Top10Degree std / Top10 Degree mean ratio}} & $\bar d=n^{-1}\sum_i d_i;\quad \sigma_d=\sqrt{n^{-1}\sum_i(d_i-\bar d)^2};\quad Q_{10}=\bar d_{top10}/\bar d$ & Average and dispersion of observed neighbors and the top-ten hub multiple. \emph{Direction:} Higher dispersion or Q10 indicates a more unequal degree distribution. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: degree / ratio}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality} \\
\textbf{Degree-centrality mean and dispersion}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: DCmean / DCstd}} & $c_D(i)=d_i/(n-1);\quad \sigma(c_D)=\sqrt{n^{-1}\sum_i(c_D(i)-\bar c_D)^2}$ & Normalized degree and cross-node dispersion used as a structural benchmark. \emph{Direction:} Higher dispersion indicates greater hub inequality. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: centrality / dispersion}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality} \\
\textbf{Weighted out- and in-strength HHI}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: weighted\_out\_degree\_hhi / weighted\_in\_degree\_hhi}} & $H^{out}=\sum_i(w_i^{out}/\sum_jw_j^{out})^2;\quad H^{in}=\sum_i(w_i^{in}/\sum_jw_j^{in})^2$ & Concentration of actor-side and beneficiary-side Pool-event weights. \emph{Direction:} Higher means more event weight is concentrated on fewer address roles. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index}} & \AVObservedTag; empirical output; no standalone visual & \cite{hirschman1964paternity} \\
\textbf{Local clustering moments and transitivity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Cluster\_mean / Cluster\_std / Transitivity}} & $C_i=2e_i/[d_i(d_i-1)];\quad T=3\times\#\text{triangles}/\#\text{connected triples}$ & Local and global closure of the undirected projection. \emph{Direction:} Higher means greater triadic closure; it does not have a universal decentralization sign. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: coefficient}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{watts1998collective} \\
\textbf{Eigenvector and closeness moments}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: eig\_mean / eig\_std / closeness\_mean / closeness\_std}} & $Ac_E=\lambda c_E;\quad c_C(i)=(n-1)/\sum_{j\neq i}d(i,j)$ & Recursive-neighbor importance and inverse geodesic distance, summarized by their mean and dispersion. \emph{Direction:} Higher dispersion indicates concentration of the stated centrality; disconnected-graph conventions must be reported. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: centrality}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality,newman2018networks} \\
\textbf{Weighted PageRank and concentration}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: maximum\_pagerank\_share / pagerank\_hhi}} & $\pi=(1-d)\mathbf 1/n+dP^\top\pi;\quad H_{PR}=\sum_i\pi_i^2$ & Stationary importance under weighted directed transitions and its concentration. \emph{Direction:} Higher HPR means PageRank mass is concentrated on fewer nodes. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score / index}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{brin1998anatomy} \\
\textbf{Community modularity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Modularity}} & $Q=(2m)^{-1}\sum_{ij}[A_{ij}-k_ik_j/(2m)]\mathbf 1\{g_i=g_j\}$ & Excess within-community connectivity relative to the configuration benchmark. \emph{Direction:} Higher means a stronger partition, not automatically more decentralization. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: score}} & \AVObservedTag; display-backbone sensitivity only; Fig.~\ref{fig:display-community-audit}; full-graph output unavailable & \cite{newman2006modularity,traag2019leiden} \\
\textbf{Core number, maximum k-core, and maximum-core share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: maximum\_k\_core / maximum\_core\_node\_share}} & $c_i=\max\{k:i\in G_k\};\quad S_{max}=n^{-1}\sum_i\mathbf 1\{c_i=k_{max}\}$ & Nested degree-based cohesion in the unweighted undirected projection. \emph{Direction:} Higher c\_i means deeper cohesion; kmax and share must be read together. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node shell / count / share}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{batagelj2003cores} \\
\textbf{Borgatti--Everett binary core and fit}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: cp\_test\_pvalue / cp\_significance / core\_cnt / avg\_core\_neighbor}} & $B_{ij}=\mathbf 1\{B_i=1\ \lor\ B_j=1\};\quad \rho_{BE}=\operatorname{corr}(A_{ij},B_{ij})$ & Fits a dense core with core--periphery ties and sparse periphery--periphery ties; the audit requires at least two core nodes. \emph{Direction:} Larger fit means closer agreement with the binary ideal; core count is definition-sensitive. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: binary node class / fit}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{borgatti2000models,kojaku2018core} \\
\textbf{Rombach continuous coreness}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: continuous coreness robustness}} & $R_{\alpha\beta}=\sum_{ij}A_{ij}C_iC_j;\quad CS_i\propto\sum_{\alpha,\beta}C_i(\alpha,\beta)R_{\alpha\beta}$ & Quality-weighted continuous coreness aggregated over the documented alpha-beta grid. \emph{Direction:} Higher means a stronger continuous core position under this definition. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score in [0,1]}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{rombach2014core} \\
\textbf{Temporal maximum-core persistence}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: persistent coreness}} & $P_i^{core}=\frac{\sum_t\mathbf 1\{c_{it}=k_{max,t}\}}{\sum_t\mathbf 1\{i\in V_t\}}$ & Fraction of a node's active topology weeks spent in that week's maximum k-core. \emph{Direction:} Higher means a more persistent address-role core position. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{holme2012temporal} \\
\textbf{Betweenness brokerage}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: brokerage}} & $b_i=\sum_{s\neq i\neq t}\sigma_{st}(i)/\sigma_{st}$ & Share of shortest paths between other nodes that pass through i. \emph{Direction:} Higher means greater geodesic brokerage under the chosen path weights. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality} \\
\textbf{Temporal community persistence}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: community persistence}} & $P_g^{comm}=\max_h |C_{g,t}\cap C_{h,t+1}|/|C_{g,t}\cup C_{h,t+1}|$ & Best adjacent-period Jaccard match for a detected community. \emph{Direction:} Higher means more stable community membership, conditional on the algorithm. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVPendingTag; no reported output; no standalone visual & \cite{holme2012temporal,traag2019leiden} \\
\textbf{Network multiplier centrality and structural HHI}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: structural\_hhi}} & $z=(I-\alpha G)^{-1}\mathbf 1;\quad H_z=\sum_i(z_i/\sum_jz_j)^2$ & Model-implied amplification of activity through network complementarities and its concentration. \emph{Direction:} Higher Hz means multiplier influence is more concentrated. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: model score / index}} & \AVSimulatedTag; simulated data; Fig.~\ref{fig:simulation-outcomes} & \cite{ballester2006keyplayer} \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Infrastructure decentralization}} \\
\textbf{Route HHI and effective routes}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: route\_hhi}} & $H_R=\sum_k q_k^2;\quad N_R^{eff}=1/H_R$ & Concentration of verified interchain activity across independent routes. \emph{Direction:} Higher HR means greater route concentration; higher effective routes means more dispersion. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index / effective route count}} & \AVSimulatedTag/\AVUnavailableTag; simulated data only; Fig.~\ref{fig:simulation-outcomes} (simulation) & \cite{belchior2021survey} \\
\textbf{Bridge or facilitator share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: bridge/facilitator shares}} & $q_k=x_k/\sum_jx_j$ & Share of verified interchain activity assigned to infrastructure k. \emph{Direction:} Higher maximum share means greater single-infrastructure dependence. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVUnavailableTag; no verified route table; no standalone visual & \cite{belchior2021survey} \\
\textbf{Targeted route-removal loss}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: max\_route\_removal\_loss}} & $L_k=(X-X^{(-k)})/X$ & Fraction of feasible activity lost when infrastructure k and its dependent links are removed. \emph{Direction:} Higher means greater functional dependence on k. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVSimulatedTag/\AVUnavailableTag; simulated data only; Fig.~\ref{fig:simulation-outcomes} (simulation) & \cite{albert2000error} \\
\textbf{Edge-disjoint route redundancy}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: disjoint paths}} & $\lambda_{uv}=\max\{\text{pairwise edge-disjoint }u\!\to\!v\text{ paths}\}$ & Number of independently edged routes between relevant layers or endpoints. \emph{Direction:} Higher means more topological redundancy, conditional on verified route edges. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: path count}} & \AVUnavailableTag; no verified route table; no standalone visual & \cite{ford1956maximal} \\
\textbf{Minimum cut}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: minimum cut}} & $\kappa_{uv}=\min_{S:u\in S,v\notin S}\sum_{e\in\delta(S)}w_e$ & Smallest verified route capacity whose removal separates u and v. \emph{Direction:} Higher means greater cut-based redundancy. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: capacity or edge count}} & \AVUnavailableTag; no verified route table; no standalone visual & \cite{ford1956maximal} \\
\textbf{Expected infrastructure-failure loss}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: expected route loss}} & $\mathcal L=\sum_k\pi_kL_k$ & Failure-probability-weighted activity loss across infrastructure components. \emph{Direction:} Higher means greater expected infrastructure exposure. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: expected share}} & \AVDiagnosticTag; no reported output; no standalone visual & \cite{acemoglu2015systemic} \\
\addlinespace[2pt]
\end{longtable}
\begin{minipage}{0.98\linewidth}
\footnotesize\emph{Notes:} ``Observed'' means a reported empirical result at the stated address or address-role unit; it does not establish an economic-actor or causal claim. ``Simulated'' denotes the mechanism simulation only. ``Pending'' includes additional benchmarks that are derivable from the documented event rows but are not reported in this study. ``Unavailable'' means the necessary verified entity, multilayer, or route-event input does not exist. A missing standalone figure does not imply missing data; the evidence status and data source remain explicit in the glossary.
\end{minipage}
\endgroup
\resumerefereelines
\end{landscape}



==> release/tables/tabA_arbitrum_gnosis_anticipation.tex <==
\begin{table}[!ht]
\centering
\caption{Sensitivity to the excluded anticipation window.}
\label{tab:arbitrum-gnosis-anticipation}
\AVTableSetup
\begin{tabularx}{0.98\linewidth}{P{0.24\linewidth}*{4}{>{\centering\arraybackslash}X}}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Excluded pre-event weeks} & \textbf{DiD-style change} & \textbf{cITS level at week 0} & \textbf{cITS slope change/week} \\
\midrule
Log participation & None & +1.3414 & +0.1551 & $-0.1158$ \\
 & 4 weeks & +1.6935 & +0.9104 & $-0.0531$ \\
 & 8 weeks (primary) & +1.9833 & +4.0396 & +0.1845 \\
\midrule
Position-holder-event HHI & None & +0.00595 & +0.06308 & +0.00350 \\
 & 4 weeks & $-0.00747$ & +0.04635 & +0.00221 \\
 & 8 weeks (primary) & $-0.01842$ & $-0.02849$ & $-0.00352$ \\
\bottomrule
\end{tabularx}
\begin{minipage}{0.96\linewidth}
\AVTableNoteFont\emph{Notes:} Direct empirical robustness output. Event week 0 is excluded in every specification; the post-period ends at week $+16$. Expanding the anticipation exclusion shortens the clean pre-period from weeks $-16{:}-1$ to $-16{:}-9$. The sensitivity, including sign changes in the controlled-ITS terms and the HHI mean-change contrast, reinforces the need to treat the estimates as comparative longitudinal evidence rather than as identified causal effects.
\end{minipage}
\end{table}


==> release/tables/tabA_arbitrum_gnosis_diagnostics.tex <==
% Values reproduced by scripts/generate_arbitrum_gnosis_comparison.py.
\begin{table}[!ht]
\centering
\caption{Differential pre-trends and pre-period placebo contrasts.}
\label{tab:arbitrum-gnosis-diagnostics}
\AVTableSetup
\begin{tabular}{llrrr}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Diagnostic} & \textbf{Estimate} & \textbf{Lower} & \textbf{Upper} \\
\midrule
Log participation & gap slope/week & -0.17259 & -0.22020 & -0.12498 \\
Position-holder-event HHI & gap slope/week & +0.00190 & 0.00034 & 0.00347 \\
\midrule
Log participation & placebo week -13 & -0.2975 & -- & -- \\
Log participation & placebo week -12 & -0.2298 & -- & -- \\
Log participation & placebo week -11 & -0.4950 & -- & -- \\
Position-holder-event HHI & placebo week -13 & -0.00720 & -- & -- \\
Position-holder-event HHI & placebo week -12 & +0.00327 & -- & -- \\
Position-holder-event HHI & placebo week -11 & +0.02075 & -- & -- \\
\bottomrule
\end{tabular}
\begin{minipage}{0.96\linewidth}
\AVTableNoteFont\emph{Notes:} Direct empirical diagnostics. Slope ranges use Bartlett/Newey--West HAC lag 2 without a finite-sample correction. Placebos compare two weeks before and after each pseudo-event within the clean pre-period. The differential slopes and material placebo movements show that causal interpretation would require additional comparison support and trend-robust designs.
\end{minipage}
\end{table}


==> release/tables/tabA_arbitrum_gnosis_horizons.tex <==
% Values reproduced by scripts/generate_arbitrum_gnosis_comparison.py.
\begin{table}[!ht]
\centering
\caption{Descriptive contrasts across alternative post-window horizons.}
\label{tab:arbitrum-gnosis-horizons}
\AVTableSetup
\begin{tabularx}{0.98\linewidth}{>{\raggedright\arraybackslash}X*{5}{>{\centering\arraybackslash}X}}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Through week} & \textbf{Arb.} & \textbf{Gnosis} & \textbf{Diff. in changes} & \textbf{NW diagnostic} \\
\midrule
Log participation & $+8$ & +0.1967 & -1.7974 & +1.9941 & [1.5700, 2.4183] \\
Log participation & $+12$ & +0.0824 & -1.9004 & +1.9829 & [1.5968, 2.3690] \\
Log participation & $+16$ & +0.0314 & -1.9519 & +1.9833 & [1.6077, 2.3589] \\
Position-holder-event HHI & $+8$ & +0.00680 & +0.02089 & -0.01409 & [-0.02034, -0.00785] \\
Position-holder-event HHI & $+12$ & +0.00713 & +0.01940 & -0.01227 & [-0.01927, -0.00527] \\
Position-holder-event HHI & $+16$ & +0.00501 & +0.02343 & -0.01842 & [-0.02900, -0.00784] \\
\bottomrule
\end{tabularx}
\begin{minipage}{0.96\linewidth}
\AVTableNoteFont\emph{Notes:} Direct empirical robustness output. The clean pre-period remains weeks $-16$ to $-9$ for every row. Bartlett/Newey--West HAC standard errors use lag 3 and no finite-sample correction. The ranges are descriptive normal approximations, not treatment-effect confidence intervals.
\end{minipage}
\end{table}


==> release/tables/tabA_arbitrum_gnosis_its.tex <==
\begin{table}[!ht]
\centering
\caption{Controlled interrupted-time-series coefficients for the Arbitrum--Gnosis gap.}
\label{tab:arbitrum-gnosis-its}
\AVTableSetup
\begin{tabularx}{0.99\linewidth}{P{0.21\linewidth}Yrrrr}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Term} & \textbf{Estimate} & \textbf{HAC SE} & \textbf{Lower} & \textbf{Upper} \\
\midrule
Log participation & Intercept & $-0.91883$ & 0.26750 & $-1.44313$ & $-0.39453$ \\
 & Pre-gap slope/week & $-0.17259$ & 0.02429 & $-0.22020$ & $-0.12498$ \\
 & Level shift at week 0 & +4.03961 & 0.41905 & 3.21827 & 4.86094 \\
 & Slope shift/week & +0.18448 & 0.03016 & 0.12537 & 0.24359 \\
\midrule
Position-holder-event HHI & Intercept & +0.017107 & 0.011197 & $-0.004839$ & 0.039053 \\
 & Pre-gap slope/week & +0.001902 & 0.000798 & 0.000338 & 0.003466 \\
 & Level shift at week 0 & $-0.028487$ & 0.012673 & $-0.053327$ & $-0.003647$ \\
 & Slope shift/week & $-0.003515$ & 0.001078 & $-0.005628$ & $-0.001403$ \\
\bottomrule
\end{tabularx}
\begin{minipage}{0.96\linewidth}
\AVTableNoteFont\emph{Notes:} Direct empirical output. The dependent variable is the weekly Arbitrum-minus-Gnosis outcome gap. The model uses clean-pre weeks $-16$ to $-9$ and post weeks $+1$ to $+16$ ($n=24$); weeks $-8$ through 0 are omitted. Bartlett/Newey--West HAC standard errors use lag 2 and no finite-sample correction. The week-0 level is extrapolated because week 0 is excluded. Ranges are normal approximations describing model-based time-series uncertainty, not treatment-effect confidence intervals.
\end{minipage}
\end{table}


==> release/tables/tabA_network_measure_glossary.tex <==
% Generated by scripts/render_network_measure_glossary.py; do not edit by hand.
\clearpage
\suspendrefereelines
\begingroup
\setstretch{1.02}
\AVTableSetup
\setlength{\tabcolsep}{3pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\renewcommand{\arraystretch}{1.16}
\begin{longtable}{>{\raggedright\arraybackslash}p{0.235\linewidth}>{\raggedright\arraybackslash}p{0.27\linewidth}>{\raggedright\arraybackslash}p{0.425\linewidth}}
\caption{Network-measure glossary: formulas, interpretation, evidence, and visualization coverage.}
\label{tab:network-measure-glossary}\\
\toprule
\AVTableHeader
\textbf{Measure} & \textbf{Notation} & \textbf{Interpretation, evidence, and source} \\
\midrule
\endfirsthead
\multicolumn{3}{c}{\tablename\ \thetable\ (continued)}\\
\toprule
\AVTableHeader
\textbf{Measure} & \textbf{Notation} & \textbf{Interpretation, evidence, and source} \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
\AVTableSubheader
\multicolumn{3}{l}{\textbf{Participation decentralization}} \\
\textbf{Active observed participants}\par\vspace{1pt}\AVTableMeta{Source field: num\_\allowbreak{}nodes (when the node set is a period's active addresses)} & \(\displaystyle\begin{gathered}N_t=|V_t|\end{gathered}\) & Number of distinct observed position-holder addresses active in period t; not a count of people or independent economic actors. \emph{Direction:} Higher means broader observed participation, conditional on the address caveat. \par\vspace{1pt}\AVTableMeta{Unit: position-holder address} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-cross-chain}; \cite{newman2018networks} \\\\
\textbf{Entrants}\par\vspace{1pt}\AVTableMeta{Source field: new nodes} & \(\displaystyle\begin{gathered}E_t=|V_t\setminus V_{t-1}|\end{gathered}\) & Addresses active in period t but not in t-1. \emph{Direction:} Higher means more observed address entry; it need not mean new economic actors. \par\vspace{1pt}\AVTableMeta{Unit: position-holder address} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows}; \cite{holme2012temporal} \\\\
\textbf{Exits}\par\vspace{1pt}\AVTableMeta{Source field: departing nodes} & \(\displaystyle\begin{gathered}X_t^{-}=|V_{t-1}\setminus V_t|\end{gathered}\) & Addresses active in t-1 but absent in t. \emph{Direction:} Higher means more observed address exit. \par\vspace{1pt}\AVTableMeta{Unit: position-holder address} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows}; \cite{holme2012temporal} \\\\
\textbf{Retained participants and retention rate}\par\vspace{1pt}\AVTableMeta{Source field: retained nodes} & \(\displaystyle\begin{gathered}R_t=|V_t\cap V_{t-1}|\\[-1pt] r_t=R_t/|V_{t-1}|\end{gathered}\) & Addresses appearing in two adjacent periods and their share of the prior-period set. \emph{Direction:} Higher r\_t means greater address persistence, not necessarily actor persistence. \par\vspace{1pt}\AVTableMeta{Unit: position-holder address / share} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows}; \cite{holme2012temporal} \\\\
\textbf{Effective number of participants}\par\vspace{1pt}\AVTableMeta{Source field: inverse HHI} & \(\displaystyle\begin{gathered}N^{\ast}=H^{-1}\\[-1pt] H=\sum_i s_i^2\end{gathered}\) & Number of equal-share participants that would generate the observed concentration. \emph{Direction:} Higher means a more even activity distribution. \par\vspace{1pt}\AVTableMeta{Unit: effective address count} \par\vspace{1pt}\AVObservedTag; empirical output; derived; no standalone visual; \cite{hirschman1964paternity} \\\\
\textbf{Cross-chain address-set overlap}\par\vspace{1pt}\AVTableMeta{Source field: Jaccard overlap} & \(\displaystyle\begin{gathered}J_t=\frac{|V_{E,t}\cap V_{A,t}|}{|V_{E,t}\cup V_{A,t}|}\end{gathered}\) & Overlap of Ethereum and Arbitrum position-holder-address sets at the same chain-relative event week. \emph{Direction:} Higher means more repeated addresses across panels; because calendar dates differ it is not contemporaneous migration. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVObservedTag; empirical output; no standalone visual; \cite{jaccard1901distribution} \\\\
\textbf{Multilayer participation coefficient}\par\vspace{1pt}\AVTableMeta{Source field: cross-layer participation} & \(\displaystyle\begin{gathered}P_i=1-\sum_{\ell}(k_{i\ell}/k_i)^2\end{gathered}\) & Dispersion of node i's connections across network layers. \emph{Direction:} Higher means connections are spread across more layers. \par\vspace{1pt}\AVTableMeta{Unit: node score in [0,1]} \par\vspace{1pt}\AVUnavailableTag; no reported output; no standalone visual; \cite{kivela2014multilayer} \\\\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{3}{l}{\textbf{Activity distribution}} \\
\textbf{Total observed activity}\par\vspace{1pt}\AVTableMeta{Source field: total\_\allowbreak{}value /\allowbreak{} event\_\allowbreak{}count} & \(\displaystyle\begin{gathered}X_t=\sum_i x_{it}\end{gathered}\) & Total action count in the empirical panels or equilibrium activity in the simulation; heterogeneous token amounts are not summed across reserves. \emph{Direction:} Scale measure, not a decentralization score by itself. \par\vspace{1pt}\AVTableMeta{Unit: events or model activity} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:simulation-outcomes}; \cite{newman2018networks} \\\\
\textbf{Pool-event-frequency Herfindahl--Hirschman index}\par\vspace{1pt}\AVTableMeta{Source field: activity\_\allowbreak{}hhi} & \(\displaystyle\begin{gathered}H_t=\sum_i s_{it}^2\\[-1pt] s_{it}=x_{it}/\sum_jx_{jt}\end{gathered}\) & Squared-share concentration of equally weighted Pool events assigned to the stated observed unit. \emph{Direction:} Higher means greater event-frequency concentration; address HHI is not actor HHI or value concentration. \par\vspace{1pt}\AVTableMeta{Unit: index in [1/n,1]} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-cross-chain}, Fig.~\ref{fig:real-v4-partial-identification}; \cite{hirschman1964paternity} \\\\
\textbf{Economic-actor HHI period bounds and change envelope}\par\vspace{1pt}\AVTableMeta{Source field: entity-adjusted HHI} & \(\displaystyle\begin{gathered}H_t^a\leq H_t^g\leq1\\[-1pt] \mathcal B_\Delta\subseteq[H_1^a-1,1-H_0^a]\end{gathered}\) & Period-specific actor-HHI bounds are sharp; subscripts 0 and 1 denote pre and post periods. Subtracting them gives a conservative outer envelope unless one common controller partition is optimized jointly. \emph{Direction:} An outer envelope crossing zero does not prove that both signs are jointly feasible. \par\vspace{1pt}\AVTableMeta{Unit: period bounds / outer envelope} \par\vspace{1pt}\AVBoundedTag; partial-identification output; Fig.~\ref{fig:real-v4-partial-identification}; \cite{molinari2020partial,binette2022entity} \\\\
\textbf{Normalized Shannon entropy}\par\vspace{1pt}\AVTableMeta{Source field: entropy} & \(\displaystyle\begin{gathered}S_t=-\frac{\sum_i s_{it}\log s_{it}}{\log n_t}\end{gathered}\) & Evenness of the activity-share distribution. \emph{Direction:} Higher means more even activity. \par\vspace{1pt}\AVTableMeta{Unit: index in [0,1]} \par\vspace{1pt}\AVPendingTag; derivable; not reported; no standalone visual; \cite{shannon1948theory} \\\\
\textbf{Gini coefficient}\par\vspace{1pt}\AVTableMeta{Source field: activity\_\allowbreak{}gini} & \(\displaystyle\begin{gathered}D_t=\sum_{ij}|x_{it}-x_{jt}|\\[-1pt] G_t=D_t/(2n_tX_t)\end{gathered}\) & Mean pairwise inequality in observed activity; the numerator aggregates pairwise absolute differences and the activity total provides the normalization. \emph{Direction:} Higher means greater inequality. \par\vspace{1pt}\AVTableMeta{Unit: index in [0,1]} \par\vspace{1pt}\AVObservedTag; empirical output; no standalone visual; \cite{gini1912variabilita} \\\\
\textbf{Top-p activity share}\par\vspace{1pt}\AVTableMeta{Source field: top1pct\_\allowbreak{}share /\allowbreak{} top10pct\_\allowbreak{}share} & \(\displaystyle\begin{gathered}T_{p,t}=\sum_{j=1}^{\lceil pn_t\rceil}s_{(j)t}\end{gathered}\) & Share held by the largest p fraction of observed units; p is 1\% or 10\% in the analysis panel. \emph{Direction:} Higher means greater top-tail concentration. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVObservedTag; empirical output; no standalone visual; \cite{newman2018networks} \\\\
\textbf{Minimum 51\% coalition}\par\vspace{1pt}\AVTableMeta{Source field: nakamoto\_\allowbreak{}51} & \(\displaystyle\begin{gathered}S_{k,t}=\sum_{j=1}^{k}s_{(j)t}\\[-1pt] \mathcal K_t=\{k:S_{k,t}\geq.51\}\\[-1pt] K_{.51,t}=\min\mathcal K_t\end{gathered}\) & Smallest number of observed units whose cumulative ordered share reaches 51\%; the calligraphic K indexed by t is the admissible threshold set. \emph{Direction:} Higher means control of the measured activity is spread across more units. \par\vspace{1pt}\AVTableMeta{Unit: address count} \par\vspace{1pt}\AVObservedTag; empirical output; no standalone visual; \cite{zhang2022sokdecentralization} \\\\
\textbf{Chain concentration}\par\vspace{1pt}\AVTableMeta{Source field: chain\_\allowbreak{}hhi} & \(\displaystyle\begin{gathered}H_{\ell}=\sum_{\ell}s_{\ell}^{2}\end{gathered}\) & Concentration of activity across chain layers. \emph{Direction:} Higher means activity is concentrated on fewer chains. \par\vspace{1pt}\AVTableMeta{Unit: index} \par\vspace{1pt}\AVSimulatedTag; simulated data; Fig.~\ref{fig:simulation-outcomes}; \cite{kivela2014multilayer} \\\\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{3}{l}{\textbf{Network structure}} \\
\textbf{Graph nodes and edges}\par\vspace{1pt}\AVTableMeta{Source field: num\_\allowbreak{}nodes /\allowbreak{} num\_\allowbreak{}edges} & \(\displaystyle\begin{gathered}n=|V|\\[-1pt] m=|E|\end{gathered}\) & Size of the address-role graph and number of unique observed ties. \emph{Direction:} Scale measures; neither alone ranks decentralization. \par\vspace{1pt}\AVTableMeta{Unit: nodes / edges} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery}; \cite{newman2018networks} \\\\
\textbf{Graph density}\par\vspace{1pt}\AVTableMeta{Source field: Relative degree} & \(\displaystyle\begin{gathered}\delta_G=\chi m/[n(n-1)]\\[-1pt] \chi\in\{1,2\}\end{gathered}\) & Fraction of possible ties that are observed; chi equals 1 for a directed graph and 2 for an undirected graph. \emph{Direction:} Direction is context-dependent; density normally falls mechanically as sparse graphs grow. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVPendingTag; derivable; not reported; no standalone visual; \cite{newman2018networks} \\\\
\textbf{Weak components and giant-component share}\par\vspace{1pt}\AVTableMeta{Source field: Components\_\allowbreak{}cnt /\allowbreak{} giant\_\allowbreak{}com\_\allowbreak{}ratio} & \(\displaystyle\begin{gathered}C=|\mathcal C(G)|\\[-1pt] g=|V^{\star}|/n\end{gathered}\) & Number of disconnected weak components and the fraction of nodes in the largest one; the component family is C(G) and the largest node set is V-star. \emph{Direction:} Larger g means greater reachability; it is not necessarily greater decentralization. \par\vspace{1pt}\AVTableMeta{Unit: count / share} \par\vspace{1pt}\AVObservedTag; giant share reported; no standalone visual; \cite{newman2018networks} \\\\
\textbf{Directed reciprocity}\par\vspace{1pt}\AVTableMeta{Source field: directed\_\allowbreak{}reciprocity} & \(\displaystyle\begin{gathered}r=m_{\leftrightarrow}/m\end{gathered}\) & Fraction of directed edges that participate in a reciprocated dyad. \emph{Direction:} Higher means more bidirectional address-role interaction; economic meaning depends on edge semantics. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVObservedTag; empirical output; no standalone visual; \cite{garlaschelli2004reciprocity} \\\\
\textbf{Degree moments and top-hub ratio}\par\vspace{1pt}\AVTableMeta{Source field: Degree mean /\allowbreak{} Degree std /\allowbreak{} Top10Degree mean /\allowbreak{} Top10Degree std /\allowbreak{} Top10 Degree mean ratio} & \(\displaystyle\begin{gathered}\bar d=n^{-1}\sum_i d_i\\[-1pt] \sigma_d^2=n^{-1}\sum_i(d_i-\bar d)^2\\[-1pt] Q_{10}=\bar d_{10}/\bar d\end{gathered}\) & Average and dispersion of observed neighbors and the top-ten hub multiple; d-bar-10 is the mean degree of the ten highest-degree nodes. \emph{Direction:} Higher dispersion or Q10 indicates a more unequal degree distribution. \par\vspace{1pt}\AVTableMeta{Unit: degree / ratio} \par\vspace{1pt}\AVPendingTag; derivable; not reported; no standalone visual; \cite{freeman1979centrality} \\\\
\textbf{Degree-centrality mean and dispersion}\par\vspace{1pt}\AVTableMeta{Source field: DCmean /\allowbreak{} DCstd} & \(\displaystyle\begin{gathered}c_i^d=d_i/(n-1)\\[-1pt] \sigma_c^2=n^{-1}\sum_i(c_i^d-\bar c)^2\end{gathered}\) & Normalized degree and cross-node dispersion used as a structural benchmark. \emph{Direction:} Higher dispersion indicates greater hub inequality. \par\vspace{1pt}\AVTableMeta{Unit: centrality / dispersion} \par\vspace{1pt}\AVPendingTag; derivable; not reported; no standalone visual; \cite{freeman1979centrality} \\\\
\textbf{Weighted out- and in-strength HHI}\par\vspace{1pt}\AVTableMeta{Source field: weighted\_\allowbreak{}out\_\allowbreak{}degree\_\allowbreak{}hhi /\allowbreak{} weighted\_\allowbreak{}in\_\allowbreak{}degree\_\allowbreak{}hhi} & \(\displaystyle\begin{gathered}p_i^{\rightarrow}=w_i^{\rightarrow}/\sum_jw_j^{\rightarrow}\\[-1pt] H^{\rightarrow}=\sum_i(p_i^{\rightarrow})^2\\[-1pt] p_i^{\leftarrow}=w_i^{\leftarrow}/\sum_jw_j^{\leftarrow}\\[-1pt] H^{\leftarrow}=\sum_i(p_i^{\leftarrow})^2\end{gathered}\) & Concentration of action-side and position-holder-side Pool-event weights; the arrowed quantities are the corresponding normalized strength shares. \emph{Direction:} Higher means more event weight is concentrated on fewer address roles. \par\vspace{1pt}\AVTableMeta{Unit: index} \par\vspace{1pt}\AVObservedTag; empirical output; no standalone visual; \cite{hirschman1964paternity} \\\\
\textbf{Local clustering moments and transitivity}\par\vspace{1pt}\AVTableMeta{Source field: Cluster\_\allowbreak{}mean /\allowbreak{} Cluster\_\allowbreak{}std /\allowbreak{} Transitivity} & \(\displaystyle\begin{gathered}C_i=2e_i/[d_i(d_i-1)]\\[-1pt] T=3\Delta_G/\Lambda_G\end{gathered}\) & Local and global closure of the undirected projection; Delta-G counts triangles and Lambda-G counts connected triples. \emph{Direction:} Higher means greater triadic closure; it does not have a universal decentralization sign. \par\vspace{1pt}\AVTableMeta{Unit: coefficient} \par\vspace{1pt}\AVPendingTag; derivable; not reported; no standalone visual; \cite{watts1998collective} \\\\
\textbf{Eigenvector and closeness moments}\par\vspace{1pt}\AVTableMeta{Source field: eig\_\allowbreak{}mean /\allowbreak{} eig\_\allowbreak{}std /\allowbreak{} closeness\_\allowbreak{}mean /\allowbreak{} closeness\_\allowbreak{}std} & \(\displaystyle\begin{gathered}A\mathbf c=\lambda_1\mathbf c\\[-1pt] c_i^{\ell}=(n-1)/\sum_{j\neq i}d_{ij}\end{gathered}\) & Recursive-neighbor importance and inverse geodesic distance, summarized by their mean and dispersion. \emph{Direction:} Higher dispersion indicates concentration of the stated centrality; disconnected-graph conventions must be reported. \par\vspace{1pt}\AVTableMeta{Unit: centrality} \par\vspace{1pt}\AVPendingTag; derivable; not reported; no standalone visual; \cite{freeman1979centrality,newman2018networks} \\\\
\textbf{Weighted PageRank and concentration}\par\vspace{1pt}\AVTableMeta{Source field: maximum\_\allowbreak{}pagerank\_\allowbreak{}share /\allowbreak{} pagerank\_\allowbreak{}hhi} & \(\displaystyle\begin{gathered}\mathbf q=(1-\eta)\mathbf 1/n\\[-1pt] \boldsymbol\pi=\mathbf q+\eta P^\top\boldsymbol\pi\\[-1pt] H_{\pi}=\sum_i\pi_i^2\end{gathered}\) & Stationary importance under weighted directed transitions and its concentration; eta is the damping parameter and q is the teleport vector. \emph{Direction:} Higher PageRank HHI means PageRank mass is concentrated on fewer nodes. \par\vspace{1pt}\AVTableMeta{Unit: node score / index} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery}; \cite{brin1998anatomy} \\\\
\textbf{Community modularity}\par\vspace{1pt}\AVTableMeta{Source field: Modularity} & \(\displaystyle\begin{gathered}B_{ij}=A_{ij}-k_ik_j/(2m)\\[-1pt] \delta_{ij}=\mathbf 1\{g_i=g_j\}\\[-1pt] Q=(2m)^{-1}\sum_{ij}B_{ij}\delta_{ij}\end{gathered}\) & Excess within-community connectivity relative to the configuration benchmark; the residual edge term is weighted by a binary same-community indicator. \emph{Direction:} Higher means a stronger partition, not automatically more decentralization. \par\vspace{1pt}\AVTableMeta{Unit: score} \par\vspace{1pt}\AVObservedTag; display-backbone sensitivity only; Fig.~\ref{fig:display-community-audit}; full-graph output unavailable; \cite{newman2006modularity,traag2019leiden} \\\\
\textbf{Core number, maximum k-core, and maximum-core share}\par\vspace{1pt}\AVTableMeta{Source field: maximum\_\allowbreak{}k\_\allowbreak{}core /\allowbreak{} maximum\_\allowbreak{}core\_\allowbreak{}node\_\allowbreak{}share} & \(\displaystyle\begin{gathered}c_i=\max\{k:i\in G_k\}\\[-1pt] I_i^{\star}=\mathbf 1\{c_i=k_{\star}\}\\[-1pt] S_{\star}=n^{-1}\sum_i I_i^{\star}\end{gathered}\) & Nested degree-based cohesion in the unweighted undirected projection; the maximum nonempty shell is paired with a binary membership indicator. \emph{Direction:} Higher coreness means deeper cohesion; the maximum shell and its share must be read together. \par\vspace{1pt}\AVTableMeta{Unit: node shell / count / share} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery}; \cite{batagelj2003cores} \\\\
\textbf{Borgatti--Everett binary core and fit}\par\vspace{1pt}\AVTableMeta{Source field: cp\_\allowbreak{}test\_\allowbreak{}pvalue /\allowbreak{} cp\_\allowbreak{}significance /\allowbreak{} core\_\allowbreak{}cnt /\allowbreak{} avg\_\allowbreak{}core\_\allowbreak{}neighbor} & \(\displaystyle\begin{gathered}B_{ij}=\mathbf 1\{b_i+b_j\geq1\}\\[-1pt] \rho_B=\rho(A,B)\end{gathered}\) & Fits a dense core with core--periphery ties and sparse periphery--periphery ties; the fit is the correlation between observed and ideal adjacency, and the audit requires at least two core nodes. \emph{Direction:} Larger fit means closer agreement with the binary ideal; core count is definition-sensitive. \par\vspace{1pt}\AVTableMeta{Unit: binary node class / fit} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery}; \cite{borgatti2000models,kojaku2018core} \\\\
\textbf{Rombach continuous coreness}\par\vspace{1pt}\AVTableMeta{Source field: continuous coreness robustness} & \(\displaystyle\begin{gathered}R_{\alpha\beta}=\sum_{ij}A_{ij}C_iC_j\\[-1pt] \chi_i\propto\sum_{\alpha,\beta}C_i(\alpha,\beta)R_{\alpha\beta}\end{gathered}\) & Quality-weighted continuous coreness aggregated over the documented alpha-beta grid. \emph{Direction:} Higher means a stronger continuous core position under this definition. \par\vspace{1pt}\AVTableMeta{Unit: node score in [0,1]} \par\vspace{1pt}\AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery}; \cite{rombach2014core} \\\\
\textbf{Temporal maximum-core persistence}\par\vspace{1pt}\AVTableMeta{Source field: persistent coreness} & \(\displaystyle\begin{gathered}P_i^{k}=\frac{\sum_t\mathbf 1\{c_{it}=k_{\star t}\}}{\sum_t\mathbf 1\{i\in V_t\}}\end{gathered}\) & Fraction of a node's active topology weeks spent in that week's maximum shell. \emph{Direction:} Higher means a more persistent address-role core position. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVObservedTag; empirical output; no standalone visual; \cite{holme2012temporal} \\\\
\textbf{Betweenness brokerage}\par\vspace{1pt}\AVTableMeta{Source field: brokerage} & \(\displaystyle\begin{gathered}b_i=\sum_{s\neq i\neq t}\sigma_{st}(i)/\sigma_{st}\end{gathered}\) & Share of shortest paths between other nodes that pass through i. \emph{Direction:} Higher means greater geodesic brokerage under the chosen path weights. \par\vspace{1pt}\AVTableMeta{Unit: node score} \par\vspace{1pt}\AVPendingTag; derivable; not reported; no standalone visual; \cite{freeman1979centrality} \\\\
\textbf{Temporal community persistence}\par\vspace{1pt}\AVTableMeta{Source field: community persistence} & \(\displaystyle\begin{gathered}J_{gh,t}=\frac{|C_{g,t}\cap C_{h,t+1}|}{|C_{g,t}\cup C_{h,t+1}|}\\[-1pt] P_{g,t}^{\mathcal C}=\max_h J_{gh,t}\end{gathered}\) & Best adjacent-period Jaccard match for a detected community. \emph{Direction:} Higher means more stable community membership, conditional on the algorithm. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVPendingTag; no reported output; no standalone visual; \cite{holme2012temporal,traag2019leiden} \\\\
\textbf{Network multiplier centrality and structural HHI}\par\vspace{1pt}\AVTableMeta{Source field: structural\_\allowbreak{}hhi} & \(\displaystyle\begin{gathered}z=(I-\alpha G)^{-1}\mathbf 1\\[-1pt] H_z=\sum_i(z_i/\sum_jz_j)^2\end{gathered}\) & Model-implied amplification of activity through network complementarities and its concentration. \emph{Direction:} Higher Hz means multiplier influence is more concentrated. \par\vspace{1pt}\AVTableMeta{Unit: model score / index} \par\vspace{1pt}\AVSimulatedTag; simulated data; Fig.~\ref{fig:simulation-outcomes}; \cite{ballester2006keyplayer} \\\\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{3}{l}{\textbf{Infrastructure dependence}} \\
\textbf{Route HHI and effective routes}\par\vspace{1pt}\AVTableMeta{Source field: route\_\allowbreak{}hhi} & \(\displaystyle\begin{gathered}H_R=\sum_k q_k^2\\[-1pt] N_R^{\ast}=H_R^{-1}\end{gathered}\) & Concentration of verified interchain activity across independent routes. \emph{Direction:} Higher route HHI means greater route concentration; a higher effective route count means more dispersion. \par\vspace{1pt}\AVTableMeta{Unit: index / effective route count} \par\vspace{1pt}\AVSimulatedTag\newline\AVUnavailableTag; simulated data only; Fig.~\ref{fig:simulation-outcomes} (simulation); \cite{belchior2021survey} \\\\
\textbf{Bridge or facilitator share}\par\vspace{1pt}\AVTableMeta{Source field: bridge/facilitator shares} & \(\displaystyle\begin{gathered}q_k=x_k/\sum_jx_j\end{gathered}\) & Share of verified interchain activity assigned to infrastructure k. \emph{Direction:} Higher maximum share means greater single-infrastructure dependence. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVUnavailableTag; no verified route table; no standalone visual; \cite{belchior2021survey} \\\\
\textbf{Targeted route-removal loss}\par\vspace{1pt}\AVTableMeta{Source field: max\_\allowbreak{}route\_\allowbreak{}removal\_\allowbreak{}loss} & \(\displaystyle\begin{gathered}L_k=(X-X^{(-k)})/X\end{gathered}\) & Fraction of feasible activity lost when infrastructure k and its dependent links are removed. \emph{Direction:} Higher means greater functional dependence on k. \par\vspace{1pt}\AVTableMeta{Unit: share} \par\vspace{1pt}\AVSimulatedTag\newline\AVUnavailableTag; simulated data only; Fig.~\ref{fig:simulation-outcomes} (simulation); \cite{albert2000error} \\\\
\textbf{Edge-disjoint route redundancy}\par\vspace{1pt}\AVTableMeta{Source field: disjoint paths} & \(\displaystyle\begin{gathered}\lambda_{uv}=|\mathcal P_{uv}^{\star}|\end{gathered}\) & Cardinality of a maximum family of pairwise edge-disjoint routes between the relevant endpoints. \emph{Direction:} Higher means more topological redundancy, conditional on verified route edges. \par\vspace{1pt}\AVTableMeta{Unit: path count} \par\vspace{1pt}\AVUnavailableTag; no verified route table; no standalone visual; \cite{ford1956maximal} \\\\
\textbf{Minimum cut}\par\vspace{1pt}\AVTableMeta{Source field: minimum cut} & \(\displaystyle\begin{gathered}\mathcal S_{uv}=\{S:u\in S,v\notin S\}\\[-1pt] \kappa_{uv}=\min_{S\in\mathcal S_{uv}}\sum_{e\in\delta(S)}w_e\end{gathered}\) & Smallest verified route capacity whose removal separates the two endpoints; the calligraphic set enumerates all separating node partitions. \emph{Direction:} Higher means greater cut-based redundancy. \par\vspace{1pt}\AVTableMeta{Unit: capacity or edge count} \par\vspace{1pt}\AVUnavailableTag; no verified route table; no standalone visual; \cite{ford1956maximal} \\\\
\textbf{Expected infrastructure\allowbreak-failure loss}\par\vspace{1pt}\AVTableMeta{Source field: expected route loss} & \(\displaystyle\begin{gathered}\mathcal L=\sum_k\pi_kL_k\end{gathered}\) & Failure-probability-weighted activity loss across infrastructure components. \emph{Direction:} Higher means greater expected infrastructure exposure. \par\vspace{1pt}\AVTableMeta{Unit: expected share} \par\vspace{1pt}\AVDiagnosticTag; no reported output; no standalone visual; \cite{acemoglu2015systemic} \\\\
\addlinespace[2pt]
\end{longtable}
\noindent\begin{minipage}{0.98\linewidth}
\AVTableNoteFont\emph{Notes:} ``Observed'' means a reported empirical result at the stated address or address-role unit; it does not establish an economic-actor or causal claim. ``Simulated'' denotes the mechanism simulation only. ``Pending'' includes additional benchmarks that are derivable from the documented event rows but are not reported in this study. ``Unavailable'' means the necessary verified entity, multilayer, or route-event input does not exist. A missing standalone figure does not imply missing data; the evidence status and data source remain explicit in the glossary.
\end{minipage}
\endgroup
\resumerefereelines



==> release/tables/tab_model_notation.tex <==
\begin{table}[t]
\centering
\caption{Core notation and evidence interpretation.}
\label{tab:model-notation}
\AVTableSetup
\begin{tabularx}{\textwidth}{P{0.10\textwidth}P{0.30\textwidth}P{0.28\textwidth}Y}
\toprule
Object & Mathematical role & Reader-facing interpretation & Evidence boundary \\
\midrule
$x_i$ & Nonnegative action of actor $i$ & Stylized protocol-activity intensity & Not a transaction count, token amount, or identified wallet \\
$b_i(p)$ & Direct net benefit under condition $p$ & Actor-specific access, cost, liquidity, or opportunity & Not an estimated GHO treatment effect \\
$g_{ij}$ & Weight with which $j$ enters $i$'s incentive & Directed economic influence $j\rightarrow i$ & Not automatically the observed Pool-event network \\
$\beta$ & Marginal response to weighted connected activity & Strategic-complementarity strength & Not an interest rate, probability, link count, or chain constant \\
$\kappa=\beta\rho(G)$ & Scale-normalized feedback strength & Comparable amplification condition across networks & Model parameter; not a decentralization score \\
$H_x$ & Sum of squared actor activity shares & Activity concentration & Address/entity interpretation requires separate evidence \\
$H_c$ & Sum of squared chain activity shares & Venue dispersion & Does not identify route independence or resilience \\
$L_k$ & Activity unavailable after route removal & Synthetic route/component stress loss & Not empirically estimated in this study \\
\bottomrule
\end{tabularx}
\end{table}



==> release/tables/tab_theory_evidence_bridge.tex <==
\begin{table}[t]
\centering
\caption{Theory-to-evidence bridge.}
\label{tab:theory-evidence-bridge}
\AVTableSetup
\begin{tabularx}{\textwidth}{P{0.20\textwidth}P{0.25\textwidth}P{0.29\textwidth}Y}
\toprule
Theoretical result & Simulation output & Observable empirical counterpart & Current empirical status \\
\midrule
Network amplification & Direct and indirect response, distance profile, and convergence & Active position-holder addresses, total actions, and third-party participation & Partial counterpart; direct exposure and economic-interaction links are not identified \\
Growth--concentration divergence & Total activity and activity HHI under equal-mass allocations & Holder HHI and action-side HHI reported with participation & Directly assessable at address level; mechanism remains noncausal \\
Dispersion--resilience divergence & Chain HHI, worst route loss, and shared-component loss & Chain shares and verified infrastructure-route dependencies & Venue dispersion is observable; route-removal outcome is not currently measurable \\
\bottomrule
\end{tabularx}
\end{table}



==> release/visual_style.tex <==
% Unified publication style for manuscript figures and tables.
% Keep this file lightweight so modular and flattened Springer builds agree.
% The manuscript body, captions, tables, and every live figure label use Latin
% Modern Roman.  A single manuscript-native family prevents the mixed serif/
% sans appearance that remained visible in RC6; weight, size, color, and
% spacing—not a second typeface—carry the hierarchy.
\RequirePackage{colortbl}
% Named-role palette shared by the technical clip-art family, explanatory
% figures, data charts, and tables.  Large surfaces stay quiet; saturated
% color is reserved for paths, headers, and evidence states.
\definecolor{AVInk}{HTML}{18324A}
\definecolor{AVNavy}{HTML}{18324A}
\definecolor{AVBlue}{HTML}{315EFB}
\definecolor{AVViolet}{HTML}{6D28D9}
\definecolor{AVTeal}{HTML}{14877D}
\definecolor{AVGreen}{HTML}{14877D}
\definecolor{AVLime}{HTML}{84B547}
\definecolor{AVOrange}{HTML}{D97745}
\definecolor{AVRed}{HTML}{C2413A}
\definecolor{AVSlate}{HTML}{18324A}
\definecolor{AVRule}{HTML}{CBD5E1}
\definecolor{AVLight}{HTML}{F5F7FB}
\definecolor{AVMist}{HTML}{EAF0FF}
\definecolor{AVWarm}{HTML}{FFF3EC}
\definecolor{AVLilac}{HTML}{F3EEFF}

% Referee-layout final-size type scale.  The body target is 9 pt, close enough
% to the 10.04 pt Springer body to feel native while preserving figure density.
% Secondary labels target 8.3 pt; 8 pt is the hard floor and is used only for
% compact identifiers/status notes.  Titles remain restrained at 10.2--11 pt.
\newcommand{\AVFigureFont}{\normalfont\rmfamily\fontsize{9.0}{10.7}\selectfont}
\newcommand{\AVFigureSmallFont}{\normalfont\rmfamily\fontsize{8.3}{9.9}\selectfont}
\newcommand{\AVFigureTinyFont}{\normalfont\rmfamily\fontsize{8.0}{9.4}\selectfont}
\newcommand{\AVFigureTitleFont}{\normalfont\rmfamily\fontsize{10.2}{11.8}\selectfont\bfseries}
\newcommand{\AVFigureHeroFont}{\normalfont\rmfamily\fontsize{11.0}{12.6}\selectfont\bfseries}
\newcommand{\AVStatusFont}{\normalfont\rmfamily\fontsize{8.1}{9.5}\selectfont\bfseries}
\newcommand{\AVTableFont}{\normalfont\fontsize{8.9}{10.8}\selectfont}
\newcommand{\AVTableNoteFont}{\normalfont\fontsize{8.1}{9.7}\selectfont}
\newcommand{\AVTableMeta}[1]{{\normalfont\fontsize{8.1}{9.6}\selectfont\color{AVInk}#1}}
\newcommand{\AVClipArt}[2][16mm]{%
  % Dynamic asset macro: the csname form prevents static dependency scanners
  % from mistaking the parameter token #2 for a literal missing filename.
  \csname includegraphics\endcsname[width=#1]{figures/clip_art/#2.pdf}%
}
\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}

\tikzset{
  av/card/.style={
    draw=AVRule,
    line width=0.58pt,
    rounded corners=2.3mm,
    fill=white,
    align=center,
    inner sep=3mm,
    blur shadow={shadow opacity=.10,shadow xshift=.45pt,shadow yshift=-.65pt}
  },
  av/model/.style={av/card,draw=AVBlue!72,fill=AVMist},
  av/observed/.style={av/card,draw=AVTeal!78,fill=AVTeal!5},
  av/descriptive/.style={av/card,draw=AVViolet!72,fill=AVLilac},
  av/risk/.style={av/card,draw=AVOrange!85,fill=AVWarm},
  av/planned/.style={av/card,draw=AVViolet!75,dashed,fill=AVLilac},
  av/unavailable/.style={av/card,draw=AVSlate,dashed,fill=AVSlate!5},
  av/hero/.style={rounded corners=3mm,draw=AVBlue!80,line width=.9pt,
    shade,top color=AVViolet!88,bottom color=AVBlue!92,text=white,
    blur shadow={shadow opacity=.22,shadow xshift=1.0pt,shadow yshift=-1.4pt}},
  av/flow/.style={-{Latex[length=1.65mm,width=1.15mm]},line width=0.78pt,draw=AVBlue},
  av/pending-flow/.style={-{Latex[length=1.65mm,width=1.15mm]},line width=0.75pt,draw=AVSlate,dashed},
  av/tag/.style={
    rounded corners=1mm,
    inner xsep=2mm,
    inner ysep=0.7mm,
    font=\AVStatusFont,
    text=white
  },
  av/icon/.style={draw=AVBlue,line width=0.76pt,line cap=round,line join=round},
  av/icon violet/.style={av/icon,draw=AVViolet},
  av/icon teal/.style={av/icon,draw=AVTeal},
  av/icon orange/.style={av/icon,draw=AVOrange},
  av/icon slate/.style={av/icon,draw=AVSlate},
  % Reusable geometry for collision-proof charts.  Titles and legends occupy
  % separate bands; legend samples never use `node[right]`, which can let the
  % next sample intrude into a long label.
  av/panel title/.style={anchor=west,font=\AVFigureTitleFont,inner sep=0pt},
  av/legend label/.style={anchor=west,inner sep=0pt},
  av/legend sample/.style={line width=1.25pt,line cap=round},
  av/figure note/.style={anchor=west,text=AVInk,inner sep=0pt}
}

% Compact semantic header mark for literature and evidence tables. The icon is
% a genuine vector micro-scene, not an emoji or an abbreviation badge.
\newcommand{\AVInlineIcon}[2][AVBlue]{%
  \tikz[baseline=-0.55ex,scale=.30]{\pic[av/icon,draw=#1] {av/#2};}\hspace{.35em}}
\newcommand{\AVTableIcon}[2][AVBlue]{%
  \makebox[0.55cm][c]{\tikz[baseline=-0.42ex,scale=.17]{\pic[av/icon,draw=#1] {av/#2};}}}

% Original, single-stroke technical icon family.  Icons supplement explicit
% labels; they never carry an empirical claim by themselves.
\tikzset{
  pics/av/blocks/.style={code={
    \draw[pic actions] (-.45,-.18) rectangle (-.13,.14);
    \draw[pic actions] (-.16,.02) rectangle (.16,.34);
    \draw[pic actions] (.13,-.18) rectangle (.45,.14);
    \draw[pic actions] (-.13,.00)--(-.02,.08);
    \draw[pic actions] (.16,.08)--(.13,.00);
  }},
  pics/av/database/.style={code={
    \draw[pic actions] (-.43,.23) arc (180:360:.43 and .14);
    \draw[pic actions] (-.43,.23) arc (180:0:.43 and .14);
    \draw[pic actions] (-.43,.23)--(-.43,-.27);
    \draw[pic actions] (.43,.23)--(.43,-.27);
    \draw[pic actions] (-.43,-.02) arc (180:360:.43 and .14);
    \draw[pic actions] (-.43,-.27) arc (180:360:.43 and .14);
  }},
  pics/av/document/.style={code={
    \draw[pic actions,rounded corners=.4pt] (-.38,-.42) rectangle (.38,.42);
    \draw[pic actions] (-.24,.20)--(.24,.20);
    \draw[pic actions] (-.24,.02)--(.24,.02);
    \draw[pic actions] (-.24,-.16)--(.12,-.16);
  }},
  pics/av/network/.style={code={
    \draw[pic actions] (-.34,.20)--(.02,-.29)--(.37,.18)--(-.34,.20);
    \draw[pic actions] (-.34,.20) circle (.09);
    \draw[pic actions] (.02,-.29) circle (.09);
    \draw[pic actions] (.37,.18) circle (.09);
  }},
  pics/av/chart/.style={code={
    \draw[pic actions] (-.43,-.35)--(-.43,.38);
    \draw[pic actions] (-.43,-.35)--(.43,-.35);
    \draw[pic actions] (-.28,-.28) rectangle (-.14,-.02);
    \draw[pic actions] (-.06,-.28) rectangle (.08,.17);
    \draw[pic actions] (.16,-.28) rectangle (.30,.34);
  }},
  pics/av/filter/.style={code={
    \draw[pic actions] (-.45,.35)--(.45,.35)--(.14,-.03)--(.14,-.36);
    \draw[pic actions] (.14,-.36)--(-.14,-.24)--(-.14,-.03)--cycle;
  }},
  pics/av/users/.style={code={
    \draw[pic actions] (0,.18) circle (.13);
    \draw[pic actions] (-.28,.09) circle (.10);
    \draw[pic actions] (.28,.09) circle (.10);
    \draw[pic actions] (-.21,-.38) arc (205:-25:.24 and .24);
    \draw[pic actions] (-.45,-.31) arc (205:-10:.17 and .16);
    \draw[pic actions] (.12,-.31) arc (190:-25:.17 and .16);
  }},
  pics/av/bridge/.style={code={
    \draw[pic actions] (-.48,-.28)--(.48,-.28);
    \draw[pic actions] (-.40,-.28)--(-.40,.32);
    \draw[pic actions] (.40,-.28)--(.40,.32);
    \draw[pic actions] (-.40,.24)..controls(-.18,-.02) and (.18,-.02)..(.40,.24);
    \draw[pic actions] (-.16,.03)--(-.16,-.28);
    \draw[pic actions] (.16,.03)--(.16,-.28);
  }},
  pics/av/code/.style={code={
    \draw[pic actions] (-.08,.34)--(-.28,-.34);
    \draw[pic actions] (-.18,.18)--(-.42,0)--(-.18,-.18);
    \draw[pic actions] (.18,.18)--(.42,0)--(.18,-.18);
  }},
  pics/av/hash/.style={code={
    \draw[pic actions] (-.18,-.42)--(-.08,.42);
    \draw[pic actions] (.10,-.42)--(.20,.42);
    \draw[pic actions] (-.42,-.14)--(.42,-.14);
    \draw[pic actions] (-.42,.15)--(.42,.15);
  }},
  pics/av/clock/.style={code={
    \draw[pic actions] (0,0) circle (.42);
    \draw[pic actions] (0,0)--(0,.24);
    \draw[pic actions] (0,0)--(.20,-.12);
  }},
  pics/av/coin/.style={code={
    \draw[pic actions] (0,0) circle (.42);
    \draw[pic actions] (0,0) circle (.27);
    \draw[pic actions] (-.12,0)--(.12,0);
  }}
}

\newcommand{\AVTableSetup}{%
  \AVTableFont%
  % Table-local floor: legacy \tiny/\footnotesize metadata is normalized to
  % the same readable 8.1 pt note scale instead of becoming microtype.
  \renewcommand{\tiny}{\normalfont\fontsize{8.1}{9.6}\selectfont}%
  \renewcommand{\footnotesize}{\normalfont\fontsize{8.1}{9.6}\selectfont}%
  \renewcommand{\arraystretch}{1.28}%
  \setlength{\tabcolsep}{3.8pt}%
  \arrayrulecolor{AVRule}%
  \setlength{\aboverulesep}{0.35ex}%
  \setlength{\belowrulesep}{0.55ex}%
  \rowcolors{2}{AVMist!34}{white}%
}

% Restrained, evidence-aware table grammar.  These commands deliberately add
% hierarchy without introducing vertical rules or decorative chartjunk.
\newcommand{\AVTableHeader}{\rowcolor{AVBlue!9}}
\newcommand{\AVTableSubheader}{\rowcolor{AVTeal!8}}
\newcommand{\AVObservedTag}{{\AVStatusFont\textcolor{AVTeal}{\ensuremath{\bullet}\,Observed}}}
\newcommand{\AVVerifiedTag}{{\AVStatusFont\textcolor{AVTeal}{\ensuremath{\checkmark}\,Verified}}}
\newcommand{\AVSimulatedTag}{{\AVStatusFont\textcolor{AVBlue}{\ensuremath{\diamond}\,Simulated}}}
\newcommand{\AVPendingTag}{{\AVStatusFont\textcolor{AVViolet}{\ensuremath{\circ}\,Pending}}}
\newcommand{\AVBoundedTag}{{\AVStatusFont\textcolor{AVOrange}{\ensuremath{\subset}\,Bounded}}}
\newcommand{\AVUnavailableTag}{{\AVStatusFont\textcolor{AVInk}{\ensuremath{\times}\,Unavailable}}}
\newcommand{\AVDiagnosticTag}{{\AVStatusFont\textcolor{AVOrange}{\ensuremath{\triangle}\,Diagnostic}}}


==> tables/tab01_general_paradigm.tex <==
\begin{table*}[t]
\centering
\caption{General protocol-network decentralization analysis paradigm.}
\label{tab:general-paradigm}
\AVTableSetup
\begin{tabularx}{0.98\textwidth}{>{\centering\arraybackslash}p{1.05cm}P{0.17\textwidth}YP{0.25\textwidth}}
\toprule
\AVTableHeader
\multicolumn{2}{l}{\textbf{Stage}} & \textbf{Research object} & \textbf{Fail-closed requirement} \\
\midrule
\AVTableIcon[AVBlue]{blocks} & \textbf{Protocol scope} & Verified contracts, chains, roles, and policy clocks & Executed and observed event, not announcement alone \\
\AVTableIcon[AVBlue]{database} & \textbf{Native events} & ABI-decoded Pool logs with block, transaction, and log keys & Emitter, signature, indexed fields, and coverage agree \\
\AVTableIcon[AVViolet]{network} & \textbf{Role network} & Typed action-side $\rightarrow$ position-holder edges by week, action, reserve, and chain & Pool emitter is not silently promoted to an economic node \\
\AVTableIcon[AVTeal]{chart} & \textbf{Evidence dimensions} & Address participation, Pool-event-frequency concentration, structural influence, and infrastructure-core or route dependence & Each dimension is classified as observed, bounded, diagnostic, simulated, rejected, or unavailable \\
\AVTableIcon[AVTeal]{clock} & \textbf{Longitudinal evidence} & Symmetric panels, topology, core--periphery, and address-to-actor bounds & Descriptive change remains distinct from an identified effect \\
\AVTableIcon[AVOrange]{filter} & \textbf{Comparative design} & Common-calendar comparison series, exclusion window, and diagnostics & Pre-paths, support, and inference determine the permitted interpretation \\
\AVTableIcon[AVViolet]{code} & \textbf{Open science} & Documented inputs, analysis programs, validation checks, and evidence table & Unsupported entity, infrastructure, or causal claims are identified explicitly \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables/tab02_policy_mechanisms.tex <==
\begin{table}[t]
\caption{Institutional innovations, countervailing mechanisms, and empirical treatment rules.}
\label{tab:policy-mechanisms}
\centering
\AVTableSetup
\begin{tabularx}{\textwidth}{p{2.55cm}XX}
\toprule
\AVTableHeader
\textbf{Institutional change} & \textbf{Countervailing mechanism} & \textbf{Empirical object and evidence status} \\
\midrule
Historical \AAVE{} network & \textit{Gain:} transferable tokens and exchange access support circulation. \textit{Risk:} exchange deposit systems and specialized contracts become persistent hubs. & Ethereum transfer graph from the October 2020 migration; historical benchmark rather than a new treatment. \\
Native \GHO{} issuance & \textit{Gain:} lower payment and borrowing frictions. \textit{Risk:} facilitator approval, bucket capacity, collateral rules, and peg support concentrate control. & Ethereum reserve activation defines the study date; technical launch, first mint, and publicity remain separate records. \\
Cross-chain \GHO{} access & \textit{Gain:} lower-cost venues attract users and disperse activity. \textit{Risk:} bridges, messaging, and rate limits can create common-mode exposure. & Arbitrum reserve activation defines the study date. Technical readiness and indexed cross-chain occurrences remain validation records, not substitute treatment dates. \\
Capacity or incentive change & \textit{Gain:} a higher bucket or incentive relaxes a binding adoption constraint. \textit{Risk:} marginal activity is directed to one facilitator, pool, or route. & Event-intensity treatment; announcement, authorization, execution, and economically binding dates remain distinct. \\
Aave v4 Hub-and-Spoke & \textit{Gain:} shared liquidity improves capital efficiency. \textit{Risk:} hub accounting, credit lines, and emergency controls raise common-infrastructure importance. & External-validity case unless activation falls inside the predefined sample; never pooled silently with V3. \\
\bottomrule
\end{tabularx}
\begin{tablenotes}\footnotesize
\item \emph{Notes:} The table states mechanisms and pre-analysis timing rules, not estimated effects. A governance proposal identifies a candidate event but does not establish treatment; route-level claims require a verified route-event table.
\end{tablenotes}
\end{table}


==> tables/tab03_literature_map.tex <==
\begin{table*}[t]
\caption{Literature map and the study's incremental contribution.}
\label{tab:literature-map}
\centering
\AVTableSetup
\setlength{\tabcolsep}{3.4pt}
\begin{tabularx}{0.98\textwidth}{>{\centering\arraybackslash}p{0.66cm}P{3.05cm}P{4.15cm}Y}
\toprule
\AVTableHeader
\multicolumn{2}{l}{\textbf{Literature stream}} & \textbf{Established insight and remaining gap} & \textbf{Role in this study} \\
\midrule
\AVTableIcon[AVBlue]{blocks} & \textbf{DeFi adoption} & Network effects can accelerate adoption, while open smart-contract finance can still concentrate activity and governance. & Separates adoption from participation, transaction, structural, and infrastructure decentralization. \\
\AVTableIcon[AVViolet]{network} & \textbf{Financial-network structure} & Centrality, communities, and core--periphery structure reveal intermediation; static address graphs obscure persistence, control, and graph-scale effects. & Adds temporal role measurement, actor bounds, scale diagnostics, and explicit requirements for route-level conclusions. \\
\AVTableIcon[AVBlue]{users} & \textbf{Network games} & Complementarities can amplify heterogeneous activity responses; formation and calibration require additional evidence. & Uses a stylized fixed-network activity model as organizing intuition, not as an estimated formation mechanism. \\
\AVTableIcon[AVOrange]{bridge} & \textbf{Stablecoins and interoperability} & Stability and reach depend on collateral, liquidity, governance, bridges, messaging, and route redundancy. & Uses verified institutional clocks for measurement windows while withholding GHO-specific and route-level effects. \\
\AVTableIcon[AVViolet]{filter} & \textbf{Causal inference} & Modern difference-in-differences and synthetic controls clarify counterfactuals; event narratives alone do not. & Uses a common-calendar comparison to expose how pre-trends, support, anticipation, and inference constrain policy language. \\
\AVTableIcon[AVTeal]{code} & \textbf{Open computational research} & Public ledgers do not by themselves reproduce deployments, labels, timing choices, or algorithms. & Links source records, documented data, analysis programs, claims, and editable paper figures through transparent supplementary materials. \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables/tab04_model_predictions.tex <==
\begin{table}[t]
\caption{Model implications, observable tests, and current validation status.}
\label{tab:model-predictions}
\centering
\AVTableSetup
\begin{tabularx}{\textwidth}{P{2.35cm}P{3.55cm}P{4.0cm}Y}
\toprule
\AVTableHeader
\textbf{Mechanism} & \textbf{Model implication} & \textbf{Observable test} & \textbf{Status} \\
\midrule
Network multiplier & A benefit shock propagates along walks in $G$; multiplier-central nodes respond more strongly. & Compare event responses by pre-policy centrality and persistent coreness. & Mechanism simulated; heterogeneity test planned. \\
Distributional incidence & Total activity can rise while $H_x$ rises or falls, depending on who receives marginal gains. & Estimate breadth and concentration jointly, by pre-treatment share and role. & Descriptive directions observed; causal effect pending. \\
Cross-chain divergence & Chain HHI can fall while dependence on a common route rises. & Report chain dispersion with route HHI and targeted-removal loss. & Chain-relative outcomes observed; route layer unavailable. \\
Route redundancy & Dividing exposure across independent routes lowers maximum single-route loss. & Compare verified route redundancy and stress removal under alternative definitions. & Simulation result only; empirical route table unavailable. \\
\bottomrule
\end{tabularx}
\begin{tablenotes}\AVTableNoteFont
\item \emph{Notes:} “Observed” denotes descriptive address-level evidence, not a causal or entity-level result. Proposed and unavailable analyses remain outside the paper's current claim set.
\end{tablenotes}
\end{table}


==> tables/tab06_pilot_did.tex <==
% Generated by scripts/run_real_v5_pilot_did.py; do not edit by hand.
\begin{table}[htbp]
\centering
\caption{Two-chain event-aligned difference-in-changes pilot (diagnostic, not causal).}
\label{tab:pilot-did}
\AVTableSetup
\setlength{\tabcolsep}{2.6pt}
\begin{tabularx}{\linewidth}{Yrrrr}
\toprule
\AVTableHeader
\textbf{Outcome} & \textbf{Ethereum} & \textbf{Arbitrum} &
\textbf{Arb. $-$ Eth.} & \textbf{NW(4) interval} \\
\midrule
\shortstack[l]{$\log(1+N_t^{p})$\\position-holder addresses} & +0.653 & +0.002 & -0.651 & [-1.002, -0.299] \\
\shortstack[l]{Position-holder\\event HHI} & -0.00301 & +0.00542 & +0.00843 & [+0.00339, +0.01347] \\
\bottomrule
\end{tabularx}
\begin{tablenotes}[flushleft]
\AVTableNoteFont
\item \emph{Notes:} For the first outcome, $N_t^{p}$ is the number of
active position-holder addresses. Entries compare mean outcome changes from event weeks $-16$ to $-1$
and $+1$ to $+16$, omitting week zero. Each chain is aligned to its own activation in a
different calendar period, and both chains receive different protocol shocks. The
interaction is Arbitrum minus Ethereum. Newey--West lag-4 intervals describe serial
variation in the paired event-week gap only; with two treated units they do not provide
valid chain-cluster causal inference. No entry is a treatment effect.
\end{tablenotes}
\end{table}


==> tables/tab07_network_measure_glossary.tex <==
% Generated by scripts/render_network_measure_glossary.py; do not edit by hand.
\begin{landscape}
\suspendrefereelines
\begingroup
\setstretch{1}
\AVTableSetup
\setlength{\tabcolsep}{3pt}
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\renewcommand{\arraystretch}{1.12}
\begin{longtable}{>{\raggedright\arraybackslash}p{3.0cm}>{\raggedright\arraybackslash}p{4.5cm}>{\raggedright\arraybackslash}p{7.1cm}>{\raggedright\arraybackslash}p{5.0cm}>{\centering\arraybackslash}p{1.3cm}}
\caption{Network-measure glossary: formulas, interpretation, evidence, and visualization coverage.}
\label{tab:network-measure-glossary}\\
\toprule
\AVTableHeader
\textbf{Indicator} & \textbf{Formula} & \textbf{Definition and direction} & \textbf{Evidence, data, and visual} & \textbf{Ref.} \\
\midrule
\endfirsthead
\multicolumn{5}{c}{\tablename\ \thetable\ (continued)}\\
\toprule
\AVTableHeader
\textbf{Indicator} & \textbf{Formula} & \textbf{Definition and direction} & \textbf{Evidence, data, and visual} & \textbf{Ref.} \\
\midrule
\endhead
\midrule
\multicolumn{5}{r}{Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Participation decentralization}} \\
\textbf{Active observed participants}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: num\_nodes (when the node set is a period's active addresses)}} & $N_t=|V_t|$ & Number of distinct observed beneficiary addresses active in period t; not a count of people or independent economic actors. \emph{Direction:} Higher means broader observed participation, conditional on the address caveat. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-cross-chain} & \cite{newman2018networks} \\
\textbf{Entrants}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: new nodes}} & $E_t=|V_t\setminus V_{t-1}|$ & Addresses active in period t but not in t-1. \emph{Direction:} Higher means more observed address entry; it need not mean new economic actors. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address}} & \AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows} & \cite{holme2012temporal} \\
\textbf{Exits}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: departing nodes}} & $X_t^{exit}=|V_{t-1}\setminus V_t|$ & Addresses active in t-1 but absent in t. \emph{Direction:} Higher means more observed address exit. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address}} & \AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows} & \cite{holme2012temporal} \\
\textbf{Retained participants and retention rate}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: retained nodes}} & $R_t=|V_t\cap V_{t-1}|;\quad r_t=R_t/|V_{t-1}|$ & Addresses appearing in two adjacent periods and their share of the prior-period set. \emph{Direction:} Higher r\_t means greater address persistence, not necessarily actor persistence. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: beneficiary address / share}} & \AVObservedTag; empirical output; Fig.~\ref{fig:address-state-flows} & \cite{holme2012temporal} \\
\textbf{Effective number of participants}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: inverse HHI}} & $N_{eff}=1/H;\quad H=\sum_i s_i^2$ & Number of equal-share participants that would generate the observed concentration. \emph{Direction:} Higher means a more even activity distribution. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: effective address count}} & \AVObservedTag; empirical output; derived; no standalone visual & \cite{hirschman1964paternity} \\
\textbf{Cross-chain address-set overlap}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Jaccard overlap}} & $J_t=|V_{E,t}\cap V_{A,t}|/|V_{E,t}\cup V_{A,t}|$ & Overlap of Ethereum and Arbitrum beneficiary-address sets at the same chain-relative event week. \emph{Direction:} Higher means more repeated addresses across panels; because calendar dates differ it is not contemporaneous migration. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{jaccard1901distribution} \\
\textbf{Multilayer participation coefficient}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: cross-layer participation}} & $P_i=1-\sum_{\ell}(k_{i\ell}/k_i)^2$ & Dispersion of node i's connections across network layers. \emph{Direction:} Higher means connections are spread across more layers. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score in [0,1]}} & \AVUnavailableTag; no reported output; no standalone visual & \cite{kivela2014multilayer} \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Transaction decentralization}} \\
\textbf{Total observed activity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: total\_value / event\_count}} & $X_t=\sum_i x_{it}$ & Total action count in the empirical panels or equilibrium activity in the simulation; heterogeneous token amounts are not summed across reserves. \emph{Direction:} Scale measure, not a decentralization score by itself. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: events or model activity}} & \AVObservedTag; empirical output; Fig.~\ref{fig:simulation-outcomes} & \cite{newman2018networks} \\
\textbf{Activity Herfindahl--Hirschman index}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: activity\_hhi}} & $H_t=\sum_i s_{it}^2;\quad s_{it}=x_{it}/\sum_jx_{jt}$ & Squared-share concentration of actions assigned to the stated observed unit. \emph{Direction:} Higher means greater concentration; address HHI is not actor HHI. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index in [1/n,1]}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-cross-chain}, Fig.~\ref{fig:real-v4-partial-identification} & \cite{hirschman1964paternity} \\
\textbf{Economic-actor HHI identified set}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: entity-adjusted HHI}} & $H_A\leq H_G\leq1;\quad \Delta H_G\in[H_{post}-1,1-H_{pre}]$ & Bounds actor-level concentration over all partitions allowed by the stated controller assumptions. \emph{Direction:} A set crossing zero does not identify the direction of the change. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: identified interval}} & \AVBoundedTag; partial-identification output; Fig.~\ref{fig:real-v4-partial-identification} & \cite{molinari2020partial,binette2022entity} \\
\textbf{Normalized Shannon entropy}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: entropy}} & $S_t=-\sum_i s_{it}\log s_{it}/\log n_t$ & Evenness of the activity-share distribution. \emph{Direction:} Higher means more even activity. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index in [0,1]}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{shannon1948theory} \\
\textbf{Gini coefficient}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: activity\_gini}} & $G_t=\frac{\sum_i\sum_j|x_{it}-x_{jt}|}{2n_t\sum_i x_{it}}$ & Mean pairwise inequality in observed activity. \emph{Direction:} Higher means greater inequality. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index in [0,1]}} & \AVObservedTag; empirical output; no standalone visual & \cite{gini1912variabilita} \\
\textbf{Top-p activity share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: top1pct\_share / top10pct\_share}} & $T_{p,t}=\sum_{j=1}^{\lceil pn_t\rceil}s_{(j)t}$ & Share held by the largest p fraction of observed units; p is 1\% or 10\% in the analysis panel. \emph{Direction:} Higher means greater top-tail concentration. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{newman2018networks} \\
\textbf{Minimum 51\% coalition}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: nakamoto\_51}} & $K_{.51,t}=\min\{k:\sum_{j=1}^{k}s_{(j)t}\geq0.51\}$ & Smallest number of observed units whose ordered activity shares reach 51\%. \emph{Direction:} Higher means control of the measured activity is spread across more units. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: address count}} & \AVObservedTag; empirical output; no standalone visual & \cite{zhang2022sokdecentralization} \\
\textbf{Chain concentration}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: chain\_hhi}} & $H_{chain}=\sum_{\ell}s_{\ell}^{2}$ & Concentration of activity across chain layers. \emph{Direction:} Higher means activity is concentrated on fewer chains. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index}} & \AVSimulatedTag; simulated data; Fig.~\ref{fig:simulation-outcomes} & \cite{kivela2014multilayer} \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Structural decentralization}} \\
\textbf{Graph nodes and edges}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: num\_nodes / num\_edges}} & $n=|V|;\quad m=|E|$ & Size of the address-role graph and number of unique observed ties. \emph{Direction:} Scale measures; neither alone ranks decentralization. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: nodes / edges}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{newman2018networks} \\
\textbf{Graph density}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Relative degree}} & $D=m/[n(n-1)]\ \text{(directed)};\quad D=2m/[n(n-1)]\ \text{(undirected)}$ & Fraction of possible ties that are observed under the declared graph direction. \emph{Direction:} Direction is context-dependent; density normally falls mechanically as sparse graphs grow. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{newman2018networks} \\
\textbf{Weak components and giant-component share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Components\_cnt / giant\_com\_ratio}} & $C=|\operatorname{comp}(G)|;\quad g=|V_{max}|/n$ & Number of disconnected weak components and the fraction of nodes in the largest one. \emph{Direction:} Larger g means greater reachability; it is not necessarily greater decentralization. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: count / share}} & \AVObservedTag; giant share reported; no standalone visual & \cite{newman2018networks} \\
\textbf{Directed reciprocity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: directed\_reciprocity}} & $r=m_{\leftrightarrow}/m$ & Fraction of directed edges that participate in a reciprocated dyad. \emph{Direction:} Higher means more bidirectional address-role interaction; economic meaning depends on edge semantics. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{garlaschelli2004reciprocity} \\
\textbf{Degree moments and top-hub ratio}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Degree mean / Degree std / Top10Degree mean / Top10Degree std / Top10 Degree mean ratio}} & $\bar d=n^{-1}\sum_i d_i;\quad \sigma_d=\sqrt{n^{-1}\sum_i(d_i-\bar d)^2};\quad Q_{10}=\bar d_{top10}/\bar d$ & Average and dispersion of observed neighbors and the top-ten hub multiple. \emph{Direction:} Higher dispersion or Q10 indicates a more unequal degree distribution. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: degree / ratio}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality} \\
\textbf{Degree-centrality mean and dispersion}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: DCmean / DCstd}} & $c_D(i)=d_i/(n-1);\quad \sigma(c_D)=\sqrt{n^{-1}\sum_i(c_D(i)-\bar c_D)^2}$ & Normalized degree and cross-node dispersion used as a structural benchmark. \emph{Direction:} Higher dispersion indicates greater hub inequality. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: centrality / dispersion}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality} \\
\textbf{Weighted out- and in-strength HHI}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: weighted\_out\_degree\_hhi / weighted\_in\_degree\_hhi}} & $H^{out}=\sum_i(w_i^{out}/\sum_jw_j^{out})^2;\quad H^{in}=\sum_i(w_i^{in}/\sum_jw_j^{in})^2$ & Concentration of actor-side and beneficiary-side Pool-event weights. \emph{Direction:} Higher means more event weight is concentrated on fewer address roles. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index}} & \AVObservedTag; empirical output; no standalone visual & \cite{hirschman1964paternity} \\
\textbf{Local clustering moments and transitivity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Cluster\_mean / Cluster\_std / Transitivity}} & $C_i=2e_i/[d_i(d_i-1)];\quad T=3\times\#\text{triangles}/\#\text{connected triples}$ & Local and global closure of the undirected projection. \emph{Direction:} Higher means greater triadic closure; it does not have a universal decentralization sign. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: coefficient}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{watts1998collective} \\
\textbf{Eigenvector and closeness moments}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: eig\_mean / eig\_std / closeness\_mean / closeness\_std}} & $Ac_E=\lambda c_E;\quad c_C(i)=(n-1)/\sum_{j\neq i}d(i,j)$ & Recursive-neighbor importance and inverse geodesic distance, summarized by their mean and dispersion. \emph{Direction:} Higher dispersion indicates concentration of the stated centrality; disconnected-graph conventions must be reported. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: centrality}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality,newman2018networks} \\
\textbf{Weighted PageRank and concentration}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: maximum\_pagerank\_share / pagerank\_hhi}} & $\pi=(1-d)\mathbf 1/n+dP^\top\pi;\quad H_{PR}=\sum_i\pi_i^2$ & Stationary importance under weighted directed transitions and its concentration. \emph{Direction:} Higher HPR means PageRank mass is concentrated on fewer nodes. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score / index}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{brin1998anatomy} \\
\textbf{Community modularity}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: Modularity}} & $Q=(2m)^{-1}\sum_{ij}[A_{ij}-k_ik_j/(2m)]\mathbf 1\{g_i=g_j\}$ & Excess within-community connectivity relative to the configuration benchmark. \emph{Direction:} Higher means a stronger partition, not automatically more decentralization. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: score}} & \AVObservedTag; display-backbone sensitivity only; Fig.~\ref{fig:display-community-audit}; full-graph output unavailable & \cite{newman2006modularity,traag2019leiden} \\
\textbf{Core number, maximum k-core, and maximum-core share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: maximum\_k\_core / maximum\_core\_node\_share}} & $c_i=\max\{k:i\in G_k\};\quad S_{max}=n^{-1}\sum_i\mathbf 1\{c_i=k_{max}\}$ & Nested degree-based cohesion in the unweighted undirected projection. \emph{Direction:} Higher c\_i means deeper cohesion; kmax and share must be read together. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node shell / count / share}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{batagelj2003cores} \\
\textbf{Borgatti--Everett binary core and fit}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: cp\_test\_pvalue / cp\_significance / core\_cnt / avg\_core\_neighbor}} & $B_{ij}=\mathbf 1\{B_i=1\ \lor\ B_j=1\};\quad \rho_{BE}=\operatorname{corr}(A_{ij},B_{ij})$ & Fits a dense core with core--periphery ties and sparse periphery--periphery ties; the audit requires at least two core nodes. \emph{Direction:} Larger fit means closer agreement with the binary ideal; core count is definition-sensitive. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: binary node class / fit}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{borgatti2000models,kojaku2018core} \\
\textbf{Rombach continuous coreness}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: continuous coreness robustness}} & $R_{\alpha\beta}=\sum_{ij}A_{ij}C_iC_j;\quad CS_i\propto\sum_{\alpha,\beta}C_i(\alpha,\beta)R_{\alpha\beta}$ & Quality-weighted continuous coreness aggregated over the documented alpha-beta grid. \emph{Direction:} Higher means a stronger continuous core position under this definition. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score in [0,1]}} & \AVObservedTag; empirical output; Fig.~\ref{fig:real-v5-core-periphery} & \cite{rombach2014core} \\
\textbf{Temporal maximum-core persistence}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: persistent coreness}} & $P_i^{core}=\frac{\sum_t\mathbf 1\{c_{it}=k_{max,t}\}}{\sum_t\mathbf 1\{i\in V_t\}}$ & Fraction of a node's active topology weeks spent in that week's maximum k-core. \emph{Direction:} Higher means a more persistent address-role core position. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVObservedTag; empirical output; no standalone visual & \cite{holme2012temporal} \\
\textbf{Betweenness brokerage}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: brokerage}} & $b_i=\sum_{s\neq i\neq t}\sigma_{st}(i)/\sigma_{st}$ & Share of shortest paths between other nodes that pass through i. \emph{Direction:} Higher means greater geodesic brokerage under the chosen path weights. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: node score}} & \AVPendingTag; derivable; not reported; no standalone visual & \cite{freeman1979centrality} \\
\textbf{Temporal community persistence}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: community persistence}} & $P_g^{comm}=\max_h |C_{g,t}\cap C_{h,t+1}|/|C_{g,t}\cup C_{h,t+1}|$ & Best adjacent-period Jaccard match for a detected community. \emph{Direction:} Higher means more stable community membership, conditional on the algorithm. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVPendingTag; no reported output; no standalone visual & \cite{holme2012temporal,traag2019leiden} \\
\textbf{Network multiplier centrality and structural HHI}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: structural\_hhi}} & $z=(I-\alpha G)^{-1}\mathbf 1;\quad H_z=\sum_i(z_i/\sum_jz_j)^2$ & Model-implied amplification of activity through network complementarities and its concentration. \emph{Direction:} Higher Hz means multiplier influence is more concentrated. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: model score / index}} & \AVSimulatedTag; simulated data; Fig.~\ref{fig:simulation-outcomes} & \cite{ballester2006keyplayer} \\
\addlinespace[2pt]
\AVTableSubheader
\multicolumn{5}{l}{\textbf{Infrastructure decentralization}} \\
\textbf{Route HHI and effective routes}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: route\_hhi}} & $H_R=\sum_k q_k^2;\quad N_R^{eff}=1/H_R$ & Concentration of verified interchain activity across independent routes. \emph{Direction:} Higher HR means greater route concentration; higher effective routes means more dispersion. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: index / effective route count}} & \AVSimulatedTag/\AVUnavailableTag; simulated data only; Fig.~\ref{fig:simulation-outcomes} (simulation) & \cite{belchior2021survey} \\
\textbf{Bridge or facilitator share}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: bridge/facilitator shares}} & $q_k=x_k/\sum_jx_j$ & Share of verified interchain activity assigned to infrastructure k. \emph{Direction:} Higher maximum share means greater single-infrastructure dependence. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVUnavailableTag; no verified route table; no standalone visual & \cite{belchior2021survey} \\
\textbf{Targeted route-removal loss}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: max\_route\_removal\_loss}} & $L_k=(X-X^{(-k)})/X$ & Fraction of feasible activity lost when infrastructure k and its dependent links are removed. \emph{Direction:} Higher means greater functional dependence on k. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: share}} & \AVSimulatedTag/\AVUnavailableTag; simulated data only; Fig.~\ref{fig:simulation-outcomes} (simulation) & \cite{albert2000error} \\
\textbf{Edge-disjoint route redundancy}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: disjoint paths}} & $\lambda_{uv}=\max\{\text{pairwise edge-disjoint }u\!\to\!v\text{ paths}\}$ & Number of independently edged routes between relevant layers or endpoints. \emph{Direction:} Higher means more topological redundancy, conditional on verified route edges. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: path count}} & \AVUnavailableTag; no verified route table; no standalone visual & \cite{ford1956maximal} \\
\textbf{Minimum cut}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: minimum cut}} & $\kappa_{uv}=\min_{S:u\in S,v\notin S}\sum_{e\in\delta(S)}w_e$ & Smallest verified route capacity whose removal separates u and v. \emph{Direction:} Higher means greater cut-based redundancy. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: capacity or edge count}} & \AVUnavailableTag; no verified route table; no standalone visual & \cite{ford1956maximal} \\
\textbf{Expected infrastructure-failure loss}\par\vspace{1pt}{\tiny\textcolor{AVSlate}{Source field: expected route loss}} & $\mathcal L=\sum_k\pi_kL_k$ & Failure-probability-weighted activity loss across infrastructure components. \emph{Direction:} Higher means greater expected infrastructure exposure. \par\vspace{1pt}{\tiny\textcolor{AVSlate}{Unit: expected share}} & \AVDiagnosticTag; no reported output; no standalone visual & \cite{acemoglu2015systemic} \\
\addlinespace[2pt]
\end{longtable}
\begin{minipage}{0.98\linewidth}
\footnotesize\emph{Notes:} ``Observed'' means a reported empirical result at the stated address or address-role unit; it does not establish an economic-actor or causal claim. ``Simulated'' denotes the mechanism simulation only. ``Pending'' includes additional benchmarks that are derivable from the documented event rows but are not reported in this study. ``Unavailable'' means the necessary verified entity, multilayer, or route-event input does not exist. A missing standalone figure does not imply missing data; the evidence status and data source remain explicit in the glossary.
\end{minipage}
\endgroup
\resumerefereelines
\end{landscape}


==> visual_style.tex <==
% Unified publication style for manuscript figures and tables.
% Keep this file lightweight so modular and flattened Springer builds agree.
% The manuscript body, captions, tables, and every live figure label use Latin
% Modern Roman.  A single manuscript-native family prevents the mixed serif/
% sans appearance that remained visible in RC6; weight, size, color, and
% spacing—not a second typeface—carry the hierarchy.
\RequirePackage{colortbl}
% Named-role palette shared by the technical clip-art family, explanatory
% figures, data charts, and tables.  Large surfaces stay quiet; saturated
% color is reserved for paths, headers, and evidence states.
\definecolor{AVInk}{HTML}{18324A}
\definecolor{AVNavy}{HTML}{18324A}
\definecolor{AVBlue}{HTML}{315EFB}
\definecolor{AVViolet}{HTML}{6D28D9}
\definecolor{AVTeal}{HTML}{14877D}
\definecolor{AVGreen}{HTML}{14877D}
\definecolor{AVLime}{HTML}{84B547}
\definecolor{AVOrange}{HTML}{D97745}
\definecolor{AVRed}{HTML}{C2413A}
\definecolor{AVSlate}{HTML}{18324A}
\definecolor{AVRule}{HTML}{CBD5E1}
\definecolor{AVLight}{HTML}{F5F7FB}
\definecolor{AVMist}{HTML}{EAF0FF}
\definecolor{AVWarm}{HTML}{FFF3EC}
\definecolor{AVLilac}{HTML}{F3EEFF}

% Referee-layout final-size type scale.  The body target is 9 pt, close enough
% to the 10.04 pt Springer body to feel native while preserving figure density.
% Secondary labels target 8.3 pt; 8 pt is the hard floor and is used only for
% compact identifiers/status notes.  Titles remain restrained at 10.2--11 pt.
\newcommand{\AVFigureFont}{\normalfont\rmfamily\fontsize{9.0}{10.7}\selectfont}
\newcommand{\AVFigureSmallFont}{\normalfont\rmfamily\fontsize{8.3}{9.9}\selectfont}
\newcommand{\AVFigureTinyFont}{\normalfont\rmfamily\fontsize{8.0}{9.4}\selectfont}
\newcommand{\AVFigureTitleFont}{\normalfont\rmfamily\fontsize{10.2}{11.8}\selectfont\bfseries}
\newcommand{\AVFigureHeroFont}{\normalfont\rmfamily\fontsize{11.0}{12.6}\selectfont\bfseries}
\newcommand{\AVStatusFont}{\normalfont\rmfamily\fontsize{8.1}{9.5}\selectfont\bfseries}
\newcommand{\AVTableFont}{\normalfont\fontsize{8.9}{10.8}\selectfont}
\newcommand{\AVTableNoteFont}{\normalfont\fontsize{8.1}{9.7}\selectfont}
\newcommand{\AVTableMeta}[1]{{\normalfont\fontsize{8.1}{9.6}\selectfont\color{AVInk}#1}}
\newcommand{\AVClipArt}[2][16mm]{%
  % Dynamic asset macro: the csname form prevents static dependency scanners
  % from mistaking the parameter token #2 for a literal missing filename.
  \csname includegraphics\endcsname[width=#1]{figures/clip_art/#2.pdf}%
}
\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}

\tikzset{
  av/card/.style={
    draw=AVRule,
    line width=0.58pt,
    rounded corners=2.3mm,
    fill=white,
    align=center,
    inner sep=3mm,
    blur shadow={shadow opacity=.10,shadow xshift=.45pt,shadow yshift=-.65pt}
  },
  av/model/.style={av/card,draw=AVBlue!72,fill=AVMist},
  av/observed/.style={av/card,draw=AVTeal!78,fill=AVTeal!5},
  av/descriptive/.style={av/card,draw=AVViolet!72,fill=AVLilac},
  av/risk/.style={av/card,draw=AVOrange!85,fill=AVWarm},
  av/planned/.style={av/card,draw=AVViolet!75,dashed,fill=AVLilac},
  av/unavailable/.style={av/card,draw=AVSlate,dashed,fill=AVSlate!5},
  av/hero/.style={rounded corners=3mm,draw=AVBlue!80,line width=.9pt,
    shade,top color=AVViolet!88,bottom color=AVBlue!92,text=white,
    blur shadow={shadow opacity=.22,shadow xshift=1.0pt,shadow yshift=-1.4pt}},
  av/flow/.style={-{Latex[length=1.65mm,width=1.15mm]},line width=0.78pt,draw=AVBlue},
  av/pending-flow/.style={-{Latex[length=1.65mm,width=1.15mm]},line width=0.75pt,draw=AVSlate,dashed},
  av/tag/.style={
    rounded corners=1mm,
    inner xsep=2mm,
    inner ysep=0.7mm,
    font=\AVStatusFont,
    text=white
  },
  av/icon/.style={draw=AVBlue,line width=0.76pt,line cap=round,line join=round},
  av/icon violet/.style={av/icon,draw=AVViolet},
  av/icon teal/.style={av/icon,draw=AVTeal},
  av/icon orange/.style={av/icon,draw=AVOrange},
  av/icon slate/.style={av/icon,draw=AVSlate},
  % Reusable geometry for collision-proof charts.  Titles and legends occupy
  % separate bands; legend samples never use `node[right]`, which can let the
  % next sample intrude into a long label.
  av/panel title/.style={anchor=west,font=\AVFigureTitleFont,inner sep=0pt},
  av/legend label/.style={anchor=west,inner sep=0pt},
  av/legend sample/.style={line width=1.25pt,line cap=round},
  av/figure note/.style={anchor=west,text=AVInk,inner sep=0pt}
}

% Compact semantic header mark for literature and evidence tables. The icon is
% a genuine vector micro-scene, not an emoji or an abbreviation badge.
\newcommand{\AVInlineIcon}[2][AVBlue]{%
  \tikz[baseline=-0.55ex,scale=.30]{\pic[av/icon,draw=#1] {av/#2};}\hspace{.35em}}
\newcommand{\AVTableIcon}[2][AVBlue]{%
  \makebox[0.55cm][c]{\tikz[baseline=-0.42ex,scale=.17]{\pic[av/icon,draw=#1] {av/#2};}}}

% Original, single-stroke technical icon family.  Icons supplement explicit
% labels; they never carry an empirical claim by themselves.
\tikzset{
  pics/av/blocks/.style={code={
    \draw[pic actions] (-.45,-.18) rectangle (-.13,.14);
    \draw[pic actions] (-.16,.02) rectangle (.16,.34);
    \draw[pic actions] (.13,-.18) rectangle (.45,.14);
    \draw[pic actions] (-.13,.00)--(-.02,.08);
    \draw[pic actions] (.16,.08)--(.13,.00);
  }},
  pics/av/database/.style={code={
    \draw[pic actions] (-.43,.23) arc (180:360:.43 and .14);
    \draw[pic actions] (-.43,.23) arc (180:0:.43 and .14);
    \draw[pic actions] (-.43,.23)--(-.43,-.27);
    \draw[pic actions] (.43,.23)--(.43,-.27);
    \draw[pic actions] (-.43,-.02) arc (180:360:.43 and .14);
    \draw[pic actions] (-.43,-.27) arc (180:360:.43 and .14);
  }},
  pics/av/document/.style={code={
    \draw[pic actions,rounded corners=.4pt] (-.38,-.42) rectangle (.38,.42);
    \draw[pic actions] (-.24,.20)--(.24,.20);
    \draw[pic actions] (-.24,.02)--(.24,.02);
    \draw[pic actions] (-.24,-.16)--(.12,-.16);
  }},
  pics/av/network/.style={code={
    \draw[pic actions] (-.34,.20)--(.02,-.29)--(.37,.18)--(-.34,.20);
    \draw[pic actions] (-.34,.20) circle (.09);
    \draw[pic actions] (.02,-.29) circle (.09);
    \draw[pic actions] (.37,.18) circle (.09);
  }},
  pics/av/chart/.style={code={
    \draw[pic actions] (-.43,-.35)--(-.43,.38);
    \draw[pic actions] (-.43,-.35)--(.43,-.35);
    \draw[pic actions] (-.28,-.28) rectangle (-.14,-.02);
    \draw[pic actions] (-.06,-.28) rectangle (.08,.17);
    \draw[pic actions] (.16,-.28) rectangle (.30,.34);
  }},
  pics/av/filter/.style={code={
    \draw[pic actions] (-.45,.35)--(.45,.35)--(.14,-.03)--(.14,-.36);
    \draw[pic actions] (.14,-.36)--(-.14,-.24)--(-.14,-.03)--cycle;
  }},
  pics/av/users/.style={code={
    \draw[pic actions] (0,.18) circle (.13);
    \draw[pic actions] (-.28,.09) circle (.10);
    \draw[pic actions] (.28,.09) circle (.10);
    \draw[pic actions] (-.21,-.38) arc (205:-25:.24 and .24);
    \draw[pic actions] (-.45,-.31) arc (205:-10:.17 and .16);
    \draw[pic actions] (.12,-.31) arc (190:-25:.17 and .16);
  }},
  pics/av/bridge/.style={code={
    \draw[pic actions] (-.48,-.28)--(.48,-.28);
    \draw[pic actions] (-.40,-.28)--(-.40,.32);
    \draw[pic actions] (.40,-.28)--(.40,.32);
    \draw[pic actions] (-.40,.24)..controls(-.18,-.02) and (.18,-.02)..(.40,.24);
    \draw[pic actions] (-.16,.03)--(-.16,-.28);
    \draw[pic actions] (.16,.03)--(.16,-.28);
  }},
  pics/av/code/.style={code={
    \draw[pic actions] (-.08,.34)--(-.28,-.34);
    \draw[pic actions] (-.18,.18)--(-.42,0)--(-.18,-.18);
    \draw[pic actions] (.18,.18)--(.42,0)--(.18,-.18);
  }},
  pics/av/hash/.style={code={
    \draw[pic actions] (-.18,-.42)--(-.08,.42);
    \draw[pic actions] (.10,-.42)--(.20,.42);
    \draw[pic actions] (-.42,-.14)--(.42,-.14);
    \draw[pic actions] (-.42,.15)--(.42,.15);
  }},
  pics/av/clock/.style={code={
    \draw[pic actions] (0,0) circle (.42);
    \draw[pic actions] (0,0)--(0,.24);
    \draw[pic actions] (0,0)--(.20,-.12);
  }},
  pics/av/coin/.style={code={
    \draw[pic actions] (0,0) circle (.42);
    \draw[pic actions] (0,0) circle (.27);
    \draw[pic actions] (-.12,0)--(.12,0);
  }}
}

\newcommand{\AVTableSetup}{%
  \AVTableFont%
  % Table-local floor: legacy \tiny/\footnotesize metadata is normalized to
  % the same readable 8.1 pt note scale instead of becoming microtype.
  \renewcommand{\tiny}{\normalfont\fontsize{8.1}{9.6}\selectfont}%
  \renewcommand{\footnotesize}{\normalfont\fontsize{8.1}{9.6}\selectfont}%
  \renewcommand{\arraystretch}{1.28}%
  \setlength{\tabcolsep}{3.8pt}%
  \arrayrulecolor{AVRule}%
  \setlength{\aboverulesep}{0.35ex}%
  \setlength{\belowrulesep}{0.55ex}%
  \rowcolors{2}{AVMist!34}{white}%
}

% Restrained, evidence-aware table grammar.  These commands deliberately add
% hierarchy without introducing vertical rules or decorative chartjunk.
\newcommand{\AVTableHeader}{\rowcolor{AVBlue!9}}
\newcommand{\AVTableSubheader}{\rowcolor{AVTeal!8}}
\newcommand{\AVObservedTag}{{\AVStatusFont\textcolor{AVTeal}{\ensuremath{\bullet}\,Observed}}}
\newcommand{\AVVerifiedTag}{{\AVStatusFont\textcolor{AVTeal}{\ensuremath{\checkmark}\,Verified}}}
\newcommand{\AVSimulatedTag}{{\AVStatusFont\textcolor{AVBlue}{\ensuremath{\diamond}\,Simulated}}}
\newcommand{\AVPendingTag}{{\AVStatusFont\textcolor{AVViolet}{\ensuremath{\circ}\,Pending}}}
\newcommand{\AVBoundedTag}{{\AVStatusFont\textcolor{AVOrange}{\ensuremath{\subset}\,Bounded}}}
\newcommand{\AVUnavailableTag}{{\AVStatusFont\textcolor{AVInk}{\ensuremath{\times}\,Unavailable}}}
\newcommand{\AVDiagnosticTag}{{\AVStatusFont\textcolor{AVOrange}{\ensuremath{\triangle}\,Diagnostic}}}

% Manuscript-native professional pseudocode box.  The code body uses the same
% Latin Modern family and >=8 pt floor as the figures and tables, while the
% numbered-line grammar remains independent of external algorithm packages.
\newcounter{avalgo}
\newcounter{avalgline}
\newenvironment{AVPseudocode}[2]{%
  \refstepcounter{avalgo}\label{#2}%
  \setcounter{avalgline}{0}%
  \begin{tcolorbox}[
    enhanced,
    breakable,
    colback=white,
    colframe=AVBlue!72,
    colbacktitle=AVMist,
    coltitle=AVInk,
    fonttitle=\AVFigureTitleFont,
    title={Algorithm~\theavalgo\enspace #1},
    boxrule=0.65pt,
    arc=1.6mm,
    left=2.3mm,
    right=2.3mm,
    top=1.7mm,
    bottom=1.7mm,
    before skip=7pt plus 2pt minus 2pt,
    after skip=7pt plus 2pt minus 2pt
  ]%
  \AVFigureSmallFont%
  \setlength{\parindent}{0pt}%
  \setlength{\parskip}{1.2pt}%
}{%
  \end{tcolorbox}%
}
\newcommand{\AVAlgLine}[1]{\par\noindent\stepcounter{avalgline}\makebox[1.45em][r]{{\AVFigureTinyFont\color{AVSlate}\arabic{avalgline}}}\hspace{0.75em}\begin{minipage}[t]{\dimexpr\linewidth-3.0em\relax}\AVFigureSmallFont #1\end{minipage}\par}
\newcommand{\AVAlgLineI}[1]{\par\noindent\stepcounter{avalgline}\makebox[1.45em][r]{{\AVFigureTinyFont\color{AVSlate}\arabic{avalgline}}}\hspace{0.75em}\begin{minipage}[t]{\dimexpr\linewidth-3.0em\relax}\AVFigureSmallFont\hspace*{1.35em}#1\end{minipage}\par}
\newcommand{\AVAlgLineII}[1]{\par\noindent\stepcounter{avalgline}\makebox[1.45em][r]{{\AVFigureTinyFont\color{AVSlate}\arabic{avalgline}}}\hspace{0.75em}\begin{minipage}[t]{\dimexpr\linewidth-3.0em\relax}\AVFigureSmallFont\hspace*{2.70em}#1\end{minipage}\par}
\newcommand{\AVAlgKeyword}[1]{\textbf{#1}}

